CASPR: Judiciously Using the Cloud for Wide-Area Packet Recovery

We revisit a classic networking problem -- how to recover from lost packets in the best-effort Internet. We propose CASPR, a system that judiciously leverages the cloud to recover from lost or delayed packets. CASPR supplements and protects best-effort connections by sending a small number of coded packets along the highly reliable but expensive cloud paths. When receivers detect packet loss, they recover packets with the help of the nearby data center, not the sender, thus providing quick and reliable packet recovery for latency-sensitive applications. Using a prototype implementation and its deployment on the public cloud and the PlanetLab testbed, we quantify the benefits of CASPR in providing fast, cost effective packet recovery. Using controlled experiments, we also explore how these benefits translate into improvements up and down the network stack.

==> ReWAN-arxiv(1)/abstract.tex <==
\begin{abstract}
 
%{\bf John:  Light-hearted abstract.  I sometimes find it helpful to write one to motivate what we really want to say here later as well as in the body.} 

We revisit a classic networking problem -- how to recover from lost packets in the best-effort Internet. 
We propose \sys{}, a system that \emph{judiciously} leverages the cloud to recover from lost or delayed packets. % with relatively low cost. 
\sys{} supplements and protects best-effort connections by sending a small number of coded packets along the highly reliable but expensive cloud paths. %with proactive transmission of encoded packets along cloud paths at a low rate.
%The encoded packets take two forms:  FEC encoding %within a stream, and network coding across parallel %streams sharing a pair of nearest-neighbor data %centers. 
When receivers detect packet loss, they recover packets with the help of the nearby data center, not the sender, thus providing quick and reliable packet recovery for latency-sensitive applications.  
%To enable a receiver to recover from a random loss, the nearby data center has useful FEC packets that it can forward, enabling recovery on sub-RTT timescales.
%To recover from burst losses, or even a sustained outage, the nearby data center enlists data from other receivers and orchestrates pipelined %collaborative recovery via network coding packets.
Using a prototype implementation and its deployment on the public cloud and the PlanetLab testbed, 
we quantify the benefits of \sys{} in providing fast, cost effective packet recovery. 
Using controlled experiments, we also explore how these benefits translate into improvements up and down the network stack. 

%Scenarios we explore include improving user %experience in video conferences over Skype, reducing %worst-case latencies in short TCP transfers, and %reducing loss in transmissions over cellular networks.

%advantages translate into   for a wide range of applications (e.g., skype, short web transfers) and network scenarios (e.g., cellular, WAN).

%in providing fast, cost-effective packet recovery for multiple latency sensitive applications (e.g., short web transfers, video conferencing). different types of applications and networks.  



%Our multi-pronged evaluation conducts microbenchmarks, demonstrates the advantages of \sys{} through experiments on both real and emulated environments,
%PlanetLab and the public cloud, 
%and shows how these benefits translate into improvements in user-perceived experience for short web transfers and Skype video conferencing. 
%a Skype video conferencing scenario. 


\begin{comment}
In today's best-effort Internet, when you fail to receive a packet, your primary recourse is to send dupacks back to your TCP sender until they eventually got around to retransmitting.  As a side-effect, they also wisely throttle their sending rate.  Emerging applications can't wait around and slow down for ``fast'' retransmissions;  they need the data now.  

The system we propose judiciously leverages the cloud to expeditiously recover from lost or delayed packets with relatively low cost.  Our system automatically supplements and protects best-effort connections with proactive transmission of low-rate encoded packets along cloud paths.  The encoded packets take two forms:  FEC encoding within a stream, and network coding across parallel streams sharing a pair of nearest-neighbor data centers. When receivers lose packets, they ping the nearby cloud data center directly, not the server.
To recover from random losses, voila: the nearby data center already has useful FEC packets. During a sustained outage, the nearby data center enlists data from other receivers and orchestrates collaborative recovery via network coding packets.  Although this has extra overhead, a connection can be maintained even when an outage on the best-effort path lasts indefinitely.
Moreover, we demonstrate that our judicious use of expensive cloud resources is much more cost-effective than other previously proposed approaches.
\end{comment}

\end{abstract}


==> ReWAN-arxiv(1)/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\sys{} seeks to connect two complementary interests: the \emph{pull} of existing (and burgeoning) applications and their demand for better user experience, and the \emph{push} of DC technology that makes cloud services more accessible to the edge than ever before. 
The key idea behind \sys{} is to use the cloud paths \emph{only} for recovery by sending coded packets across the reliable but expensive inter-DC paths. As more applications shift their services to the cloud and as highly interactive VR/AR applications continue to emerge, classical algorithmic techniques such as coding can address fresh challenges. We view \sys{} as a promising step toward providing application and network architects with new insights into how to judiciously leverage the cloud.

\newpage

%, and expect continued research in this area in the years to come.


%The main challenge for \sys{} is to satisfy three often competing constraints simultaneously: timely recovery, maximal recovery, and low %cost.

%Cross-stream coding and cooperative recovery are the key components that allow \sys{} to meet these demands. Together, they can both (1) %relieve the temporal constraints of time budgets (due to the immediate nature of recovery and straggler mitigation) and (2) recover an %indefinite series of losses on multiple paths, all while keeping costs low by taking advantage of free ingress cloud bandwidth and %judiciously using the egress bandwidth.


%, especially with regards to mobility and NFV.

==> ReWAN-arxiv(1)/design.tex <==
\section{Design}
\label{sec:design}
In this section, we first outline key design goals for a packet recovery service.% for latency sensitive applications.% has to achieve.
Next we overview \sys{}'s design and show how it meets these challenges, and then describe key components of our system in detail. Our goals are:

%In this section, we first outline key design goals that a packet recovery service for latency sensitive applications has to achieve.  Next we overview \sys{}'s design and show how it meets these challenges, and then describe key components of our system in detail.  Our goals are:


%\begin{enumerate}
   
    \paragraph{Timely packet recovery.}  Traditional retransmission mechanisms for end-to-end packet recovery necessarily incur latency overheads at the timescale of multiple RTTs. For applications with much lower latency tolerance, recovering both delayed packets as well as packets that are lost on sub-RTT timescales is a requirement.
    
     \paragraph{Maximal protection.} Traditional methods for protecting against bit errors and packet losses have limited efficacy when faced with loss bursts or %complete 
     outages. Any service should provide protection against a wide range of loss scenarios, minimizing the number of packets that are lost or excessively delayed. %While some interactive applications can tolerate a small amount of packet loss, \sys{} should still strive to minimize such events, in order to effectively handle the demands of emerging applications (e.g., Virtual Reality). 
     
    \paragraph{Low bandwidth overhead (cost).} Minimize the use of the expensive inter-DC cloud bandwidth, thus ruling out traditional overlay solutions which use the cloud path for \emph{all} of the traffic~\cite{via2016}. 
    
    %In addition to the inter-DC bandwidth, \sys{} also optimizes for the current pricing model of cloud providers which charge for egress %bandwidth while ingress bandwidth is free. 
%\end{enumerate}




\begin{comment}

    \paragraph{Timely packet recovery.}  Traditional retransmission mechanisms for end-to-end packet recovery necessarily incur latency overheads at the timescale of multiple RTTs. For applications with much lower latency tolerance, recovering both delayed packets as well as packets that are lost on sub-RTT timescales is a requirement. 
     \paragraph{Maximal protection.} Traditional methods for protecting against bit errors and packet losses have limited efficacy when faced with loss bursts or complete outages. Any service should provide protection against a wide range of loss scenarios, minimizing the number of packets that are lost or excessively delayed. %While some interactive applications can tolerate a small amount of packet loss, \sys{} should still strive to minimize such events, in order to effectively handle the demands of emerging applications (e.g., Virtual Reality). 
    \paragraph{Low bandwidth overhead (cost).} Minimize the use of the expensive inter-DC cloud bandwidth, thus ruling out traditional overlay solutions which use the cloud path for \emph{all} of the traffic~\cite{via2016}. 
\end{comment}

%Jb -- wrong place, breaks flow.
%In this section, we first provide an overview of \sys{}'s design and show how it meets these challenges. We then describe key components of our system in detail.

\begin{figure}[!t]
 \includegraphics[scale=0.5]{figures/overview-new.png}
 \caption{\sys{} Overview.}
 \label{fig:overview}
\end{figure}


\subsection{\sys{} Overview}


% Main idea of overview:
%   Overall working (all the different pieces in the system). 
%   Key aspect of coding. 
%   Key aspect of recovery protocol.
%To achieve the three design goals, \sys{} permits applications to transmit along Internet paths while supplementing those flows with coded %recovery packets along the cloud path. Therefore, the coded packets will be close to the destination and used for recovery (if needed) without %requiring a full RTT. By using the cloud path \textit{only} for coded packets, we keep bandwidth costs low while enabling timely recovery. We %further discuss the packet coding and recovery mechanisms in Sections XX and XX, but first demonstrate how \sys{} works with a simple example.

\begin{comment}
 \begin{figure}[!t]
  \centering
  \includegraphics[scale=0.50]{figures/overview-new.png}
  \label{fig:overview}
  %\subfigure[Cross-stream Coding]{\includegraphics[scale=0.40]{figures/vertical-basic2.png}\label{vertical-basic}}
  %\subfigure[In-stream Coding]{\includegraphics[scale=0.40]{figures/horizontal-basic2.png}\label{horizontal-basic}}
  \caption{\sys{} Overview.}
 % \osama{update figure labels.  jb:  these subscripts are really sloppy.  let's just color-code the packets.  also add a third coded packet on %DC1->DC2 and mark packets 1-3 as being lost on the R1->S1 path to match the example text.}
 \label{fig:overview}
 \end{figure}
\end{comment}
 
\begin{comment}
\begin{figure}[!t]
 \includegraphics[scale=0.5]{figures/overview-new.png}
 \caption{\sys{} Overview.}
 \label{fig:overview}
\end{figure}
\end{comment}


Figure~\ref{fig:overview} shows the high level workings of \sys{} through a basic example. There are two sender-receiver pairs ($S_1$-$R_1$ and $S_2$-$R_2$), %where the senders and receivers
each connected via a wide area path. For example, they may be on separate continents. There are two DCs that are running the \sys{} service: DC1 is in close physical proximity to the senders and DC2 is close to the receivers. 
The senders and receivers communicate on the wide area path using IP's best effort service, but in addition, each sender also sends a copy of each packet
%\john{Is this really only a footnote?  seems like a major assumption, needs justification.} \osama{we can move it up, also we do touch upon this in skype experiments}
to its nearby \sys{} service (DC1). 

%Given the relatively low bit rate of many latency sensitive applications, short duration of web transfers, and the increasing capacity of access links, we claim that sending a copy of the data to the cloud is feasible. \footnote{In~\S\ref{subsec:mobile-eval}, we discuss one %scenario in which this assumption may not apply and how \sys{} can potentially still provide benefits.} %In figure~\ref{fig:overview}, S1 sends packets 1, 2 \& 3 and S2 send packets 5,6 \& 7 to both destination and nearest data center (DC1).
%\footnote{Given the relatively low bit rate of many latency sensitive applications, short duration of web transfers, and the increasing capacity of access links, we claim that sending a copy of the data to the cloud is feasible. In~\S\ref{subsec:mobile-eval}, we discuss one %scenario in which this assumption may not apply and how \sys{} can potentially still provide benefits.}



\paragraph{Coding.} DC1 generates a small number of \emph{coded} packets, which are sent to the recovery service at DC2 using the inter-DC cloud path. \sys{} uses a novel \emph{cross-stream} coding design: coding is done \emph{across} a subset of user streams, which protects against bursty losses or even complete outages on a network path. For example, if ($S_1$-$R_1$) experiences an outage, \sys{} undertakes a \emph{cooperative} recovery process by combining the coded packets at DC2 with the data packets of $S_2$-$R_2$ to recover the lost packets. 
%Second, packet recovery tends to be faster compared to traditional FEC-based recovery because the timing gap between the coded packet and its %corresponding data packet is typically lower. 

The cooperative recovery process, however, has its own set of challenges. 
First, decoding overhead can be high since that involves getting data packets from all other flows in the encoding subset. 
To ensure that this procedure is invoked only when necessary, \sys{} also uses \emph{in-stream} coding,
whereby it generates a small number of FEC packets \emph{within} a single user stream, thereby avoiding the potentially costly cooperative recovery process for random losses.% (e.g., a single lost packet in a batch). 
Unlike traditional end-to-end FEC, these in-stream coded packets are transmitted along the inter-DC path. Second, during cooperative recovery, some packets could be lost or delayed, especially if many streams are involved -- we call this the \emph{straggler problem}. \sys{}'s cross-stream coding accounts for potential stragglers by generating extra coded packets, thereby treating packets from stragglers similarly to losses on the direct Internet path.  

\begin{comment}
 \begin{figure}[!t]
  \centering
  \includegraphics[scale=0.50]{figures/overview-new.png}
  \label{fig:overview}
  %\subfigure[Cross-stream Coding]{\includegraphics[scale=0.40]{figures/vertical-basic2.png}\label{vertical-basic}}
  %\subfigure[In-stream Coding]{\includegraphics[scale=0.40]{figures/horizontal-basic2.png}\label{horizontal-basic}}
  \caption{\sys{} Overview.}
 % \osama{update figure labels.  jb:  these subscripts are really sloppy.  let's just color-code the packets.  also add a third coded packet on %DC1->DC2 and mark packets 1-3 as being lost on the R1->S1 path to match the example text.}
 \label{fig:overview}
 \end{figure}
\end{comment}

\paragraph{Packet Recovery.} \sys{} uses a novel, 
receiver-driven packet recovery protocol which optimizes for
today's cloud pricing model that only charges for egress cloud bandwidth usage. Unlike traditional protocols, there is no involvement of the sender; instead, the receiver undertakes out-of-band packet recovery; it detects losses using a combination of missing sequence numbers and timeouts, and informs DC2 about any lost packets. For some packet losses, it suffices for DC2 to relay the in-stream coded packets. In other instances, the DC may need to undertake cooperative recovery, by contacting other receivers, obtaining their packets and combining them with the cross-stream coded packets to recover missing packets. Since most of the bandwidth overhead in this process is due to packets coming \emph{into} the cloud (DC2) and is thus cost-free,
we proactively use cooperative recovery after three consecutive lost packets, resulting in faster recovery for large bursty losses or outages. 

%\sys{}'s current design does not include any protection for losses experienced on $S/R$-$DC$ paths. In our real world evaluation (\S\ref{subsec:pl-eval}), we note that simple ARQ based recovery schemes on these paths will provide us with adequate protection.

\paragraph{Cost.} \sys{}'s design explicitly minimizes the bandwidth cost of using the cloud's egress bandwidth. This is reflected in two design decisions. First, \sys{} only exchanges a small number of recovery packets between DCs. This is the major difference between \sys{} and a solution that \emph{only} uses the cloud~\cite{via2016}, we also compare cost of both these solutions in ~\S\ref{subsec:prototype-eval}. Second, recovery between DC2 and the receiver is \emph{on-demand}: this saves the egress bandwidth charges at DC2, albeit at the expense of (slightly) slower recovery.
%% JB - no new para
In general, the design of \sys{} aims to explore the spectrum between exclusive use of best-effort Internet paths and exclusive use of cloud paths, striving to optimize the trade-off between wide area packet recovery and cost.


%\begin{comment}

\begin{comment}


\subsection{Design Justification}

\paragraph{Packet Duplication vs Path Switching.}
\sys{} uses packet duplication at the sender to achieve timely and maximal packet recovery. An alternative to packet duplication is a path switching scheme which only uses cloud overlay when public Internet path experiences problems. However, for low bandwidth applications, path switching has much higher overhead~\cite{andersenbest}. We further discuss how to reduce sender duplication overhead and retain the benefits of our current scheme in ~\S\ref{subsec:deployment}.


\paragraph{Number of Overlay Nodes.}
\sys{}'s use of two node overlay results in faster recovery times as receivers can perform on-demand recovery from near-by DC node. Additionally, using local retransmissions on the edge ($S/R$-$DC$) paths results in better recovery rates (\S\ref{subsec:pl-eval}).
A single DC node overlay does not provide such benefits as it is far from both or one of the end hosts.


\paragraph{Coding Scheme.}
A recent study~\cite{rewanhotnets} as well as our experiments (\S\ref{subsec:pl-eval}) show that random losses are most common on Internet but outages contribute more towards loss rate. 
Hence, \sys{} uses \emph{in-stream} for random losses and \emph{cross-stream} for bursty losses and outages.

\paragraph{Design Assumptions.}
\sys{} provides most gains if the following conditions hold. i) latency added by overlay path, coding, and packet recovery is low. ii) Losses of receiver are independent. iii) Losses on public Internet and inter-DC paths are independent.  Our evaluation (\S\ref{subsec:pl-eval},~\ref{subsec:mobile-eval},~\ref{subsec:prototype-eval}) as well as previous study~\cite{rewanhotnets} shows that these conditions hold most of the time.


\end{comment}


\begin{comment}
\subsection{Deployment Scenarios}
\label{subsec:deployment}
\osama{rework this and place full duplication in the motivation section and rest in discussion section}
A packet recovery service can be used in variety of ways: it can potentially be deployed by the cloud infrastructure provider, an ISP, or a third-party service provider who pays the cloud operator only for the infrastructure usage. Users can explicitly opt into using it if they require a more reliable packet recovery service -- for example, implemented as a paid service or added value proposition.  
The following deployment scenarios determine \emph{who} duplicates the packets (and sends them to the packet recovery service) and \emph{which} packets are duplicated. Three possible scenarios could be:


\begin{enumerate}[leftmargin=*]
    \item \emph{Full Duplication at Source.} This is the primary scenario that we focus on in this paper -- in this case, the source duplicates every packet and sends a copy to the cloud for possible recovery at a later time. 
    Given the relatively low bit rate of many latency sensitive applications, and the increasing capacity of access links, we claim that this strategy is feasible in many common scenarios. 
    Our experiments also confirm the feasibility of this approach for  a wide range of application and network scenarios, including challenging ones like the use of video conferencing over cellular networks. However, if access capacity is limited, duplication may cause edge congestion, making the next two scenarios more applicable.
    
    
    
    %While it may seem that this overhead of duplication is %excessive, we argue that it is feasible for most of %today's users. There are two main reasons for our claim. %First, many of today's latency sensitive applications have %low bandwidth demands e.g. a Skype HD call only requires %1.5Mbps~\cite{skype_bw}. Second, recent reports have shown %that global average connection speed is increasing and is %at least 7Mbps for both fixed and mobile %users~\cite{akamai_report,speedtest_report}. In fact %Akamai's recent study shows that around 82\% of global %users have at least 4Mbps connection speed with 45\% of %users having greater than 10Mbps~\cite{akamai_report}. 
    
    
    \item \emph{Selective Duplication at Source.} When full duplication at source is infeasible -- due to limited access bandwidth or high bitrate of the application -- we can use the packet recovery service 
    only for selected packets, such as an  I-frame for video streaming, important user actions for gaming or AR applications, or the last packet of a window for short TCP transfers~\cite{gentleaggression}. 
    
    %Such selective duplication can provide a lower overhead alternative to the full duplication option described earlier, and can be used in scenarios where sources have limited bandwidth or limited budget for packet recovery. 
    
    \item \emph{Duplication inside the network.} A third strategy, which requires support from the network, involves setting a bit in the packet, which indicates whether packet recovery is required or not. Based on the value of this bit, the ISP could duplicate the packet and send it to the cloud for packet recovery. Similarly, this duplication can also happen at a nearby data center, which can send the original packet through the public Internet and use the cloud path for coded packets only.
\end{enumerate}

Irrespective of which packets are duplicated and who duplicates them, the core of a packet recovery service lies in how the cloud service \emph{encodes} these packets and then subsequently \emph{recovers} them in case of a loss. 
\end{comment}
%We now present the design of our proposed packet recovery service, with a focus on these two key design elements. 





\begin{comment}

 \begin{figure}[!t]
  \centering
  \includegraphics[scale=0.50]{figures/overview-new.png}
  \label{fig:overview}
  %\subfigure[Cross-stream Coding]{\includegraphics[scale=0.40]{figures/vertical-basic2.png}\label{vertical-basic}}
  %\subfigure[In-stream Coding]{\includegraphics[scale=0.40]{figures/horizontal-basic2.png}\label{horizontal-basic}}
  \caption{\sys{} Overview.}
 % \osama{update figure labels.  jb:  these subscripts are really sloppy.  let's just color-code the packets.  also add a third coded packet on %DC1->DC2 and mark packets 1-3 as being lost on the R1->S1 path to match the example text.}
 \label{fig:overview}
 \end{figure}
\end{comment}

\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.30]{figures/overview.png}
 \caption{\sys{} overview.}
 \label{fig:overview}
\end{figure}

Figure~\ref{fig:overview} shows an environment for which \sys{} is used: two nodes, \texttt{Sender} and \texttt{Receiver}, interacting via some application across a wide area. Between them exists an Internet path as well as at least one cloud overlay path, via nodes \texttt{DC1} and \texttt{DC2}. The Internet path is practically free to use but only gives a best-effort service, and the cloud overlay path is costly but is highly available and provides low latency.

\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.22]{figures/coding.png}
 \caption{Example of coding a recovery packet.}
 \label{fig:coding}
\end{figure}

Consider a stream of packets from \texttt{Sender} flowing across the Internet path to \texttt{Receiver}. As packets leave \texttt{Sender}, they are also multicast through an access path to \texttt{DC1}. At \texttt{DC1}, groups of packets are composed using coding technologies (cite) into a coded (recovery) packet (Figure~\ref{fig:coding} ). \texttt{DC1} then transmits the recovery packet along the data center path to \texttt{DC2}.

When \texttt{Receiver} detects that packet X has been lost along the Internet path, it queries \texttt{DC2} to trigger recovery. \texttt{DC2} can then send the relevant recovery packet to \texttt{Receiver} so that it may use it to decode and recover packet X.

The use of the cloud overlay to do coding, transmission, and recovery enables \sys{} to achieve the three design goals. The coding allows \sys{} to perform recovery in the face of losses along the Internet path, and the recovery algorithm at \texttt{DC2} and \texttt{Receiver} makes the recovery quite timely, especially compared to a retransmission. Finally, \sys{} limits the egress bandwidth overhead of the overlay path by only sending recovery packets, which keeps costs low.

This simple example is only meant to illustrate the basic principles of \sys{}. Therefore, we now expand upon this setup by enriching our coding and recovery methodologies to make sure we are getting maximal, timely recovery at relatively low cost.

\end{comment}

\subsection{Coding}
\label{sec:coding}

\begin{comment}
\sys{}'s coding design faces three main challenges. We now discuss the challenges and our approach. 

\begin{enumerate}

\item Timing constraints:  for each application using our packet recovery service, a packet can only be coded together with other packets that arrive at the DC within a short time window. With the exception of applications like telephony, predicting the arrival times of packets in advance is difficult. We use a combination of offline and dynamic selection: a candidate pool of flows is selected in advance based on the location of the receivers, and within this pool, coding is done based on the packets that arrive within a short time interval.  

\item Handle a wide range of packet loss and delay scenarios, including random losses, bursty losses, and outages:
Our design thus codes both within a stream as well as across streams to provide protection against a wide range of scenarios. 

\item Deal with stragglers during cooperative recovery process: 
Our coding approach treats stragglers as additional losses and provisions enough coded packets in the cross-stream coding to account for them. 
\end{enumerate}
\end{comment}
We now elaborate the two key decisions made by the encoding process: i) deciding which batches of packets to encode over (Coding Plan) and ii) deciding how many encoded packets to generate (Coding Rate).
%% I removed the question marks -- looked weird.

\subsubsection{Coding Plan}
%In \sys{}, senders send a copy of their packets to their nearest data center, DC1, which generates different types of coded packets and sends to %nearest data center of destination, DC2.
%There are two main steps applied before generating a coded packet.

The coding plan needs to account for \emph{spatial} and \emph{temporal} constraints while forming a batch of packets on which coding will be applied. By spatial constraints, we mean that only flows with the same destination DC can be considered together for cross-stream coding. For example, if DC1 is in the Eastern US region and is receiving traffic destined for a European DC and an Asian DC, it forms two groups, one for each destination DC.
%\john{I don't understand the use of the word node in this next sentence.  Do we mean flow?  Are there lower and upper bounds on flows %per group?  Where do we record which flows belong in which group?  Can a flow belong to multiple groups (for the same destination DC, of %course)?}
Each flow belongs to one group and DC1 keeps a track of the mapping of flows to groups. 
Within a group, we pick a further subset of flows based on the arrival timing of their packets to form coding batches. 
%-- we show in Section XX that selecting flows randomly from the overall group performs almost as good as a careful selection of flows %that consider the performance history of a flow while determining the coding plan.



Temporal constraints restrict packets in a batch to only those packets that arrive within a short interval -- this imposes an encoding delay. For in-stream coding, the encoding delay is well-understood (and is considered a limitation of FEC for low bitrate applications) as we need to wait for all packets in a block to arrive before we can generate the FEC packets. However, \sys{}'s use of  cross-stream coding ensures that encoding delay is typically lower, because packets from different user streams can arrive within a short time-frame, even if each application individually is generating low bitrate traffic. Finally, our coding module limits the block size (for a given level of protection) and uses timeouts to bound delay. 
%Our scalability evaluation in Section XX shows that fixed timer values and block sizes provide us the most benefit \fahad{is this %accurate?}

%% JB:  moved forward, one pic per column
\begin{comment}


\begin{figure}[!t]
\centering
  %\hspace{-1em}
  \subfigure[\small cross-stream and\\
  in-stream encoding]{\includegraphics[width=1.13in]{figures/c1.png}\label{fig:coding-1}}
\hspace{1em}
  \subfigure[\small $Y_A$~protects~flow\\ 
  $A$ (in-stream).]{\includegraphics[width=1.0in]{figures/c2.png}\label{fig:coding-2}}
 \hspace{2em}
  \subfigure[\small $X$'s protect\\ flow $A$ (cross-stream).]{\includegraphics[width=1.0in]{figures/c3.png}\label{fig:coding-3}}
\hspace{2em}
 \subfigure[\small $X$'s protect $A$\\
 and $C$ (cross-stream).]{\includegraphics[width=1.0in]{figures/c4.png}\label{fig:coding-4}}
  \caption{Coded Packet Generation and Recovery.}
 \end{figure}

\end{comment}
%The coding module running at DC1 first groups flows together according to destinations with the same DC2.\john{How does DC1 make this %determination? by IP address? another way?} For example, if DC1 is in the Eastern US region and is receiving traffic destined
%for a European DC and an Asian DC, it will form two groups -- one for each data center -- and will place the packets in the appropriate per-group %queues for coding.
%European and Asian data centers, it will place can make two groups, one each corresponding to the destination data center (Figure~\ref{fig:cand-sel}).

%Within the same group, DC1 dynamically codes batches of packets depending on other packets present during the same time interval %(Figure~\ref{fig:code-plan}). DC1 also has fixed block sizes for coded packets along with timers for each block. \cody{Need basic coding plan, %then give details later in evaluation.}  Our scalability evaluation in section XX shows that fixed timer values and block sizes provide us the %most benefit.

 
 



\subsubsection{Coding Rate}
Given a batch of data packets arriving at DC1, \sys{} needs to decide how many cross-stream and in-stream coded packets to generate. For both types, the coded packets are created using a block code (for example, Reed-Solomon codes), which allows \sys{} to generate multiple coded packets per batch if desired.  Figure~\ref{fig:coding-1} depicts some of the possible tradeoffs, for a batch of 20 packets from four synchronous (for simplicity) flows, A-D.  In this depiction, in-stream encoding proceeds horizontally: a single FEC packet ($Y_i$) is produced for each flow $i$.  Cross-stream encoding proceeds vertically:  two cross-stream packets are produced from groups of four packets across flows, i.e., $A2$, $B2$, $C2$, and $D2$ are combined to generate coded packets $X3$ and $X4$.

Coding logically proceeds with two rates: an in-stream encoding rate of $s < 1$ coded packets per within-flow data packets, and a cross-stream encoding rate of 
$r < 1$ coded packets per data packet, where the data packets are selected among at most $k$ different flows.\footnote{We deviate from the standard notation of block coding theory, where $k$ data elements are encoded to generate a block of size $n$, yielding $(n - k)$ coded packets. Data rate and timing constraints may require us to code before $k$ packets are available.} 
Note that DC1 must also include information in the coded packets about which flows and sequence numbers are represented, to facilitate later recovery.
In our depicted setting, we have $k = 4$, $r = \frac{2}{4}$ and $s=\frac{1}{5}$, but in practice we use fewer coded packets for a batch of data packets, with the typical overhead of coded packets less than 20\%. 

Coded packets provide protection in multiple ways.  In-stream encoding packets protect primarily against random loss, much like traditional FEC.  As depicted in Figure~\ref{fig:coding-2}, packet $Y_A$ can recover from the loss of $A_3$.
Cross-stream packets protect against bursty losses or outages on the direct Internet path, and against the possibility of receivers being stragglers during cooperative recovery.
%\john{This is not good:  we haven't defined recovery yet!} Figure~\ref{fig:coding-3} demonstrate that if packets $A_2$ through $A_4$ are lost in a burst, then corresponding packets from $B$, $C$, and $D$ along with $X3$, $X5$, and $X7$ are sufficient to decode the missing packets for $A$.
In figure~\ref{fig:coding-4}, if some of $C$'s packets are also lost on the direct path, additional protection using more encoding packets could enable recovery at both $A$ and $C$.  The cooperative recovery mechanism is described in \ref{subsec:loss-recovery}.

%\begin{comment}

Our depiction begs the question: why are both types of encoding useful, and how much protection is advisable?   We view in-stream coding as a first line of defense: providing faster recovery for random losses.  Cross-stream encoding, on the other hand is both much more powerful (it can recover both random and bursty losses), but also incurs a potentially higher delay associated with recovery.
In our evaluation, we quantify these costs and weigh them against how beneficial multiple coded packets are in terms of protection from losses and decreased packet recovery times.

%\end{comment}
\begin{figure}[!t]
\centering
  \hspace{-2em}
  \subfigure[][\small cross-stream and 
  in-stream encoding]{\includegraphics[width=1.13in]{figures/c1.png}\label{fig:coding-1}}
\hspace{2em}
  \subfigure[][\small $Y_A$~protects~flow
  $A$ (in-stream).]{\includegraphics[width=1.0in]{figures/c2.png}\label{fig:coding-2}}
 \hspace{0.35em}
  \subfigure[][\small $X$'s protect flow $A$ (cross-stream).]{\includegraphics[width=1.0in]{figures/c3.png}\label{fig:coding-3}}
\hspace{2em}
 \subfigure[][\small $X$'s protect $A$
 and $C$ (cross-stream).]{\includegraphics[width=1.0in]{figures/c4.png}\label{fig:coding-4}}
  \caption{Coded Packet Generation and Recovery.}
 \end{figure}
\paragraph{Coding Parameters.} For cross-stream coding, we use a default of two cross-stream coded packets ($r = 2/k$) to mitigate the effects of stragglers and protect against bursty losses and outages.% on the direct path.%, setting $r = 2/k$. 
In practice, we bound $k$ to a moderate value ($k <= 10$ in our evaluation), since larger values add significant overhead in the cooperative recovery process. When more than $k$ flows use \sys{} concurrently at an ingress DC, the DC organizes them into subgroups of at most $k$ flows per group.

For in-stream coding, we find that for interactive applications -- where the average frame rate is 10-15 fps and the average frame is composed of 2-5 packets~\cite{chitchat} -- it is best suited to send an in-stream packet for each frame ($s=\frac{1}{5}$), although that results in relatively higher overhead, so applications with low cost budget can choose to fall back to cross-stream coding only. The in-stream encoding overhead is less for applications that send back-to-back packets, such as 
TCP flows, where a single coded packet can be sent for an entire TCP window (e.g., $s=\frac{1}{16}$ or $s=\frac{1}{32}$)

%Similarly, for short web transfers where each window has 10-20 packets, we send an in-stream packet for every 5 packets. Therefore, when we evaluate our prototype, we set $s=\frac{1}{5}$. 

%Note that in scenarios where 

% \begin{figure}[!t]
%\centering
% \includegraphics[scale=0.40]{figures/coding-plan.png}
% \caption{Example of \sys{} coding plan, only packets present at the same time are coded together.}
% \label{fig:code-plan}
%\osama{modify figure to show time}
% \end{figure}

\begin{algorithm}[!t]
\scriptsize
\SetKwFunction{KwFn}{dc1\_process(pkt, flow\_id):}
\textbf{def} \texttt{in\_stream\_qs[]}\\
\textbf{def} \texttt{cross\_stream\_qs[][]}\\
\BlankLine
\KwFn

\Indp
   \BlankLine
   \textit{// (1) In-stream coding.}\\
   \nl \texttt{q = in\_stream\_qs[flow\_id]}\\
   \nl \texttt{q.push(pkt)}\\
   \nl \If{\texttt{q.isFull()}} {
       \nl \texttt{in\_coded\_pkts = encode(q)}\\
       \nl \texttt{send(dc2\_id, in\_coded\_pkts)}\\
    }
    \BlankLine
    \textit{// (2) Cross-stream coding.}\\
    \nl \texttt{dc2\_id = extract\_dc2\_id(flow\_id)}\\
    \nl \texttt{q\_index = next\_round\_robin\_q(flow\_id)}\\
    \nl \texttt{q = cross\_stream\_qs[dc2\_id][q\_index]}\\
    \BlankLine
    \textit{// Find a queue that doesn't have a packet from this flow.}\\
    \nl \texttt{initial\_q = q}\\
    \nl \While {\texttt{q.contains(flow\_id)}} {
        \nl \texttt{q\_index = next\_round\_robin\_q(flow\_id)}\\
        \nl \texttt{q = cross\_stream\_qs[dc2\_id][q\_index]}\\
        \textit{// If we've tried all q's, empty the first by encoding or discarding.}\\
        \nl \If {\texttt{q $==$ initial\_q}} {
            \nl \If {\texttt{q.size() > 1}} {
                \nl \texttt{cross\_coded\_pkts = encode(q)}\\
                \nl \texttt{send(dc2\_id, cross\_coded\_pkts)}\\
            }
            \nl \Else {
                \nl \texttt{q.clear()}\\
            }
            \nl \texttt{\textbf{break}}\\
        }    
    }
    
    \BlankLine

    \nl \texttt{q.push(pkt)}\\
    \nl \If {\texttt{q.isFull()}} {
        \nl \texttt{cross\_coded\_pkts = encode(q)}\\
        \nl \texttt{send(dc2\_id, cross\_coded\_pkts)}\\
    }
 \caption{Coding algorithm at DC1.}
\label{alg:dc1}
\end{algorithm}
\paragraph{Coding Algorithm.}
DC1 follows Algorithm~\ref{alg:dc1}, which captures the task of encoding across multiple flows at once. DC1 maintains two sets of queues: one set for in-stream encoding (one set per flow),
%% JB - redundant
%, where we keep a queue for each flow's packets, 
and a set for cross-stream encoding (one set per $k$).
%% JB -- redundant
%, where each queue is a mix of packets from the different flows that utilize the same egress DC2 node. 
When a packet arrives, it is copied and pushed into one queue of each type. 

Lines 1-5 check whether the relevant in-stream queue has reached a threshold, and if so, create coded packets and send them to DC2. For cross-stream coding, DC1 first selects the set of queues destined for the same DC2, and then chooses the individual queue in round-robin order (lines 6-8). DC1 avoids placing multiple packets from the same flow in the same cross-stream queue; if there already exist packets from the same flow in all queues, then DC1 processes the oldest queue. If there is only a packet from the flow in question, then the old packet is evicted and discarded, since sending cross-stream packets with only packets from a single stream reduces its effectiveness (lines 9-19). Once the packet is pushed into a cross-stream queue, if a threshold is reached, then coded packets are generated and sent to DC2 (lines 20-23).
%In practice, this case can be made infrequent by setting the number of cross-stream queues sufficiently high to prevent a high-rate stream from dominating the queues,
% If there are packets from multiple flows, then that queue's packets are encoded and sent.
%% CODY:  I don't think this last bit is going to work.
%% Take one fast stream and one slow stream.
%% Fast stream puts a packet in every queue.
%% Slow stream never triggers sends.
%%
%% If a fast stream is dominating, it should drop out.
%or suppressing cross-stream coding temporarily.

%\john{we can do a lot better than linear scanning of all queues, which seems kinda lame to me.  if we do round-robin placement into queues for each flow, we will preserve the different-stream property.  to do it, we'll need a last\_queue ID for each flow that we increment after insertion.  I don't know how to do it offhand without per-flow state.}

%\cody{Round-robin doesn't exactly capture time-sensitive nature of the algorithm either. John's idea: formalize an objective function. We want to maximize the diversity of the queues (or minimize the number of duplicated flows per queue) while bounding the amount of time that packets stay in the queue.}
%\fahad{we never specify how many crossstream queues we use? Some predefined number?}


Timing constraints pose a challenge to this algorithm. If one flow is much faster than all other flows, DC1 cannot hold back recovery data from the faster flow to wait to make full recovery packets. Therefore, we create a timer for each in-stream and cross-stream queue (not shown in Algorithm~\ref{alg:dc1}). On expiry of a queue timer, DC1 encodes all packets in the queue and sends them to DC2. %For cross-stream coding, if all of the queued packets belong to the same flow at encoding time, then this transmission is suppressed (as it is equivalent to an additional in-stream encoding packet).

\subsection{Recovery Protocol}
\label{subsec:loss-recovery}
\sys{} uses a receiver-driven recovery protocol: the onus is on the receiver to quickly \emph{detect} packet loss and undertake \emph{recovery} with the help of DC2. 

%Our recovery protocol leverages well known building blocks, including NACKs based on missing sequence numbers and timeouts, and adapts %them based on the peculiar nature of our settings (e.g., need for cooperative recovery, cloud pricing model, etc). Much of the novelty %in our approach comes from how the receiver \emph{predicts} the next packet's arrival time using a simple two-state markov model, and %during the \textit{recovery} phase of the protocol, including how it decides between different types of recovery options, its use of %cooperative recovery, and optimizations for reducing spurious recoveries and to speed up recovery for bursty losses.

%In particular, we use well-known methods for fast loss \textit{detection} at the receiver, including using sequence gaps between %packets and timeouts to detect a loss, as well as using NACKs to indicate the loss to the receiver-side DC.

%\cody{We don't discuss loss detection %more until we describe what we do in the prototype in Implementation -- not sure if that is OK.}. 
%\john{I think it's fine -- resolved}


\paragraph{Loss Detection.}
The key challenge in loss detection is how to make a fast, accurate prediction of whether a packet is lost (and thus needs to be recovered using the nearby DC). 
Note that our receiver based loss detection cannot use traditional sender-based timeout mechanisms (e.g., TCP RTO) because the receiver does not have a notion of \emph{when} a particular packet is sent by the sender. 

In \sys{}, the receiver detects a loss if
%one of the following conditions is met
either a gap in sequence numbers is detected (the simple case) or a timer expires for the next expected packet. Setting a suitable timeout value -- low enough for fast recovery, but high enough not to cause spurious timeouts -- requires learning and predicting packet arrival times. While this opens up the possibilities to use machine learning algorithms, our current design uses a simple two-state Markov model that works well for our workloads.

\emph{Two-State Markov Model.} The model utilizes packet inter-arrival time probabilities (based on past packet arrival history) to switch between two timeout values: it uses a \emph{small} timeout value for packets arriving within a burst (i.e., sub-RTT scale), and a \emph{long} timeout value across packet bursts or application sessions. Initially, the receiver starts off with the long timeout value, which is a function of the RTT of the path, but as soon as it starts receiving packets with a short inter-arrival time, it switches to the small timeout value -- a value chosen based on previously observed inter-arrival times of packets within a burst. It remains in this state until the small timeout expires and switches immediately to the long timeout value after sending a NACK.  To avoid spurious recoveries at burst or session boundaries -- indicated by a NACK arriving before the corresponding coded packet -- DC2 first checks with the receiver before undertaking the recovery. 
%To reduce spurious recoveries cased by state switching, the receiver and DC synchronize before any recovery can take place. Such %synchronization is only triggered if a NACK arrives much earlier (e.g. RTT) than the actual coded packet at DC2. In such cases DC2 will %ask the receiver whether to recover the packet or not. This synchronization step exchanges small packets between DC2 and receiver, so %bandwidth overhead is low.




%\sys{}'s receiver timeout mechanism has evolved from a simple weighted moving average to a 2-state timer mechanism based on packet %arrival probabilities. We now briefly describe design of both these techniques.
%\paragraph{Weighted Moving Average Timer.} \sys{}'s initial loss detection design was based on setting a timer, $T$, calculated as:  $ %T \gets \alpha \times \lambda_{new} + (1-\alpha) \times T $, where inter-arrival times ($\lambda$) are factored in with a weight %$\alpha$. 
%While this technique works well with applications that generate constant bit rate traffic, it is difficult to tune it for applications %with variable bit rate traffic as problems with convergence and spurious recoveries require manual tuning for each path.
\begin{comment}

\paragraph{2-State Probability Timer.} \sys{}'s current loss detection method utilizes packet inter-arrival time probabilities to switch between two timeout values. It uses a primary timeout value for packets arriving within a short time span (e.g. subRTT scale) and a secondary timeout value for packets arriving after a relative long delay (e.g. RTT scale). A receiver first starts off with the secondary timeout value (e.g. RTT of the path), as soon as it starts receiving packets with a short inter-arrival time, it switches to the primary timeout value (learned from packet traces). It remains in this state until the primary timeout expires and switches immediately to secondary timeout value after sending a NACK. %Figure~ref{} shows this process.

To reduces spurious recoveries cased by state switching, we use an optimization in which a DC2 and a receiver synchronize before any recovery can take place. This case is only triggered if a NACK arrives much earlier (e.g. RTT) than the actual coded packet at DC2. In such cases DC2 will ask the receiver whether to recover the packet or not. This synchronization step exchanges small packets between DC2 and receiver, so bandwidth cost is not an issue.





The goal of the \sys{} packet recovery protocol is fast recovery from various types of losses. There are two main challenges that \sys{} faces during loss recovery: 
\begin{enumerate}
    \item Timely loss detection:
    
%%    As receivers in \sys{} depend on their
%%   nearest data center for packet recovery, the sooner a packet loss is detected, the faster the recovery takes %place. 
We make receivers responsible for detecting losses as they are best equipped to make decisions about which packet to recover. Receivers use a dynamic NACK-based timeout mechanism to detect and recover from packet loss. 
    \item Sub-RTT loss recovery:
 Once a receiver's nearest data center is notified of a loss, it initiates the appropriate type of recovery. Within-stream recovery is preferable, as it does not require further communication.  Alternatively, cross-stream
 recovery is initiated.
 \john{I don't get why we prioritize cross-stream in the below.}
 This means that not only should the data center determine which type (in-stream or cross-stream) of loss recovery packet to use, it must also have that loss recovery packet readily available. Our protocol prefers cross-stream coded packets over in-stream packets as they are readily available at the data center and can be used for faster and \cody{word choice here} better recovery. \cody{Do we always prefer it? It's more expensive.} 
\end{enumerate}
\end{comment}

\subsubsection{Loss Recovery Overview}
%In \sys{}, a receiver does not contact sender for recovering lost packet, instead, recovery is done closer to the receivers in partnership with nearby data center (DC2).
\begin{comment}
\cody{Can we add a parameter here to tune when in-stream is preferable vs. cross-stream? Have to wait longer to be more sure that in-stream is good enough, but it is less expensive.}
\john{I think we should prefer in-stream.  Provided that there is not a burst loss, and assuming FEC is sent periodically at sub-RTT intervals over the DC path, there will be a sub-RTT in-stream codeword coming to correct the loss.  This is FAR better than cross-stream.  Fail over to cross-stream when there is either a burst loss or loss on the DC->DC path.  In particular, when a receiver initiates loss recovery, it is either due to a gap or to a timeout. If it's a gap (easy), you can tell whether or not you had a burst loss -- usually not, so use in-stream.  If it's a timeout (bad), maybe the DC can infer what type of loss is happening.  Maybe default to cross-stream here, not sure.  Adjust discussion below accordingly.}
\end{comment}

Upon receiving a NACK from the receiver, DC2 must determine which loss recovery scheme is best: in-stream or cross-stream cooperative recovery.  Using a cheapest first philosophy, 
in-stream recovery from coded packets already present at DC2 is preferred. In this process, DC2 forwards the relevant in-stream coding packets to the receiver, who recovers lost data by decoding them in combination with other data packets from the stream. 



When immediate in-stream recovery is inadequate, the question of which loss recovery mechanism to pursue presents an interesting tradeoff.  If the time budget allows for it, it may be tempting to wait
to see if more in-stream coded packets or ACKs arrive at DC2, signaling that in-stream recovery is sufficient, as this is cheaper in terms of both cost (bits transmitted) and recovery. However, cooperative recovery has two advantages. Coding across streams enables us to recover from bursty losses or outages in addition to random losses, and also allows the recovery process to begin \emph{immediately}, since the data packets used for cross-stream coding (and needed for decoding) tend to have arrived at other receivers in close temporal proximity to the losses, by construction. Thus, we prioritize cross-stream decoding whenever in-stream recovery is insufficient at decision time.

%In \sys{}, cross-stream recovery is given preference over in-stream recovery as it provides better protection against bursty losses and outages. %Moreover, in-stream based recovery is dependent on the arrival of future packets at the receiver, which not only results in delayed recovery but %also might end up failing due to the bursty nature of losses on Internet paths.

%If loss is random, it might be useful to try in-stream based recovery first. However, if loss is bursty, using cross-stream recovery will provide both maximum and faster packet recovery.
%If data center decides to use cross-stream coded packet, it will slightly increase bandwidth cost due to outgoing cooperative recovery requests but packet recovery will be faster as compared to using in-stream recovery.

%In \sys{}, cross-stream recovery is given preference over in-stream based recovery. The main reason for giving cross-stream coded packets priority is the bursty nature of losses on Internet. It is highly likely that packet loss will not be random, and using in-stream based recovery will result in longer recovery times.
%\paragraph{Cooperative Recovery}
%Figure~\ref{fig:coop-recovery} illustrates an example of cross-stream-based cooperative packet recovery. There are four receivers, R1 through R4, %receiving packets through wide area Internet paths. In normal operation, acknowledgement reports (ACKs) are sent from each receiver to DC2. Then, %receiver R4 experiences a burst of losses along the Internet path. In this case, in-stream coded packets will not be of any use: if they are sent %along the direct path, they will likely also be lost, and if they are sent along the cloud path, the data packets needed to decode them will not %be available. Cooperative recovery is the only option to recover such losses in a timely manner.

%Due to this long burst of losses, the R4 NACK timer will expire and it will send NACK packets to DC2 (Figure~\ref{fig:coop1}). 
%If there are bursty losses, receiver will continue sending NACKs to DC2 until it starts receiving packets from the sender.
%Receivers send reports to DC2 to notify it of packets that have been successfully received. In cases of bursty losses or outages, timers will expire that force the receiver to send NACK packets to DC2 (Figure~\ref{fig:coop1}). This informs DC2 that there are potentially many losses occurring on the Internet path.
%For every loss that DC2 recognizes through NACKs from the receiver, it determines if the packet can be recovered using  a cross-stream coded packet or not.
%In this example, cross-stream decoding is necessary and possible, as there are no NACKS from other receiver sharing the cross-stream coded packet.
%If the necessary cross-stream coded packets are present, DC2 sends cooperative recovery requests to each of the relevant nearby receivers. These receivers look in their caches of recently-received packets and send the requested packets back to DC2 in the form of cooperative recovery responses. DC2 waits for enough of these responses to perform recovery. Potentially, it can ignore stragglers if enough cross-stream coded packets are present. It then decodes the lost packet(s) and transmits them to the lossy receiver.

\begin{comment}

\end{comment}


%The recovery algorithm itself is simple, for recovery using in-stream coded packets, data center simply sends the coded packet to receiver for decoding purposes. For recovery using cross-stream coded packets, data center sends cooperative recovery requests to other destinations specified in the coded packet. 
%Once data center receives enough packets for recovery, it generates the lost packet and sends it to the original destination.

\paragraph{Fast Cooperative Recovery.} As an optimization, we make packet recovery faster by  using a proactive loss detection mode. In this mode, if DC2 receives enough consecutive loss recovery requests (NACKs) from a receiver, it does not wait for additional NACKs, and instead proactively initiates cooperative recovery for subsequent packets in anticipation that they may also be lost. DC2 switches back to normal recovery upon receiving an ACK, once the receiver starts receiving packets on the direct path from the sender again.

\begin{comment}

%DC2 cooperative request algo
\begin{algorithm}[!t]
\scriptsize

\SetKwFunction{KwFnb}{start\_cross\_recovery(lost\_flow\_id, lost\_seqnum):}

\BlankLine
\textit{// Cross-stream coded packets, indexed by a (flow, seqnum) entry. }\\
\textbf{def} \texttt{\textbf{$cross\_stream\_pkts[][]$}}\\
\BlankLine
\BlankLine
\KwFnb
%        

\Indp
    \BlankLine
    \textit{// An entry is combination of flow ID and sequence number.}\\
    \texttt{lost\_entry $=$ (lost\_flow\_id, lost\_seqnum)}\\
    \BlankLine
    \BlankLine
    
    \textit{// Don't recover if we don't have any cross-stream packets yet or if\\ // recovery has already started.}\\
    \uIf{\texttt{cross\_stream\_pkts[lost\_entry].empty() $or$ recovery\_started(lost\_entry)}}{
        \textbf{\texttt{return}};\\
    }
    \BlankLine
    \BlankLine
    \textit{// Send cooperative request to each receiver in the coded packet.}\\

    \ForEach{\texttt{pkt in cross\_stream\_pkts[lost\_entry]}} {
        \ForEach{\texttt{rcvr\_entry in pkt}} {
            \uIf{\texttt{rcvr\_entry $!=$ lost\_entry} } {
                \texttt{send\_coop\_req(rcvr\_entry)}\\
             } \texttt{mark\_recovery\_started(rcvr\_entry)\\}
        }
    }
    \texttt{mark\_recovery\_started(lost\_entry)}
    
    
\Indm
 \caption{DC2 Cooperative Request}
 \label{alg:coop-req}
\end{algorithm}







%cooperative response algo
\begin{algorithm}[!t]
\scriptsize

\SetKwFunction{KwFna}{process\_coop\_resp(coop\_resp):}
\BlankLine
\BlankLine
\textit{// Data packets from cooperative responses.}\\
\textbf{def} \texttt{\textbf{$coop\_resp\_pkts[][]$}}\\
\BlankLine
\BlankLine
\textit{// Cross-stream coded packets. }\\
\textbf{def} \texttt{\textbf{$cross\_stream\_pkts[][]$}}\\

\BlankLine
\BlankLine
\KwFna

\Indp

    \BlankLine
    \BlankLine
    \texttt{lost\_entry $=$ extract\_entry(coop\_resp)}\\
    \BlankLine
    \textit{// We may receive cooperative responses after recovery completes, \\ // in which case we ignore them.}\\
    \uIf{\texttt{recovery\_complete(lost\_entry)}} {
        \textbf{\texttt{return}};\\
    }

    \BlankLine
    \BlankLine
    \textit{// Get already received coded packets for this lost packet.}\\
    \texttt{reco\_pkts = cross\_stream\_pkts[lost\_entry]}\\
    
    \BlankLine
    \BlankLine
    \textit{// Get already received cooperative responses for this lost \\ // packet, and add the new cooperative response packet.}\\
    \texttt{resp\_pkts = coop\_resp\_pkts[lost\_entry]}\\
    \texttt{resp\_pkts.append(coop\_resp)}\\
    
    \BlankLine
    \BlankLine
    \textit{// Check if we have enough response and recovery packets \\ // to decode the missing packet.}\\
    \texttt{missing = len(coop\_resp.flows)-len(resp\_pkts)}\\
    \uIf{\texttt{missing <= len(reco\_pkts)}} {
        \BlankLine
        \textit{// Decode the lost packets and send them.}\\
        \texttt{lost\_pkts = decode(resp\_pkts, reco\_pkts)}\\
        \texttt{send(lost\_pkts)}\\
        \texttt{mark\_recovery\_complete(lost\_entry)}\\
    }   
    
 \caption{DC2 Cooperative Response}
\label{alg:coop-resp}
\end{algorithm}

\end{comment}

\paragraph{Cooperative Recovery Algorithm.}
%We divide the cross-stream packet recovery into two parts: cooperative requests and cooperative responses.;;

 \begin{figure}[!t]
\centering
 \includegraphics[scale=0.14]{figures/coop_recovery.png}
 \caption{Cooperative Recovery.
 %% JB doesn't think we need this
 %A detected loss (at $R4$) triggers DC2 to send cooperative recovery requests to nearby receivers. Even though there may be stragglers ($R1$) in sending cooperative recovery responses, DC2 may have enough coded packets to decode the lost packet(s) to send to the lossy receiver.
 }
 \label{fig:coop_recovery}
 \end{figure}

Figure~\ref{fig:coop_recovery} shows a detailed look at the cooperative recovery protocol.
%Recall that each cross-stream coded packet contains some combination of packets from various flows, so
After receiving a NACK from receiver R4 (step 1), DC2 decides which type of recovery to use. After choosing cooperative recovery, it checks that there are sufficient cross-stream coded packets to conduct the recovery process. If so, DC2 parses each one to retrieve the addresses of the relevant receivers, and then sends cooperative requests to those receivers since they have the data packets needed to decode the missing packets (step 2). %\john{Note: if they didn't have those packets, the DC would be receiving recovery requests from them, so they truly are likely to have thosepackets.}
%Cooperative requests are only sent if the appropriate cross-stream packets exist and packet requests have not already been sent. In the rare event that another flow in the same cross-coded packet has already triggered recovery, the data is unrecoverable, and the cooperative request fails at the DC. 
%
DC2 then processes any incoming cooperative recovery responses from the solicited receivers (step 3).
%It first checks whether recovery has already been completed, since it's possible that stragglers may be responding with extra cooperative responses after recovery is done. Then,
%
%% JB we've said this several times
%All packets involved in cross-stream coding and cooperative recovery must include information about all flows involved, 
By tracking responses, DC2 can tabulate the number of cooperative responses for each recovery event. 
For each loss, once the number of responses is equal to $k - 1$ 
%is greater than or equal to the number of lost packets, \john{Is this correct?  Shouldn't it be k-1?  See e-mail},
then recovery is possible. DC2 then decodes the lost packets and sends them to the receiver (4). Depending on the number of cross-stream coded packets, DC2 may only require a few of the receivers to respond in a timely fashion, thereby ignoring stragglers (such as $R1$ in Figure~\ref{fig:coop_recovery}) that can cause delay in recovery.
%If the number of missing responses is less than or equal to the number of recovery (cross-stream coded) packets available, then decoding is possible. The lost packets are then decoded and sent to the appropriate receiver. If not enough cooperative responses have been received, DC2 waits for other receivers to respond.
Since recovery is time sensitive, the protocol fails silently if not enough coded packets or cooperative recovery responses are received within a set deadline. We discuss these conditions under which recovery is not possible in Section~\ref{sec:wide_area_results}


Repeatedly applying this cooperative recovery process not only enables \sys{} to recover an \emph{indefinite} series of losses in most circumstances, but also makes the recovery process relatively fast compared to wide area retransmissions. Since each cross-stream packet is encoded from a batch of data packets (across different flows) with similar send times, cooperative recovery can be performed immediately, as opposed to waiting to collect enough packets for decoding from a single, linear stream. This, in combination with the ability to tune the coding rate to mitigate the effects of stragglers, relieves the temporal constraints imposed by time budgets. Additionally, the acknowledgement and cooperative recovery process in \sys{} exploits the current cloud pricing model, in which all incoming traffic is free and outgoing traffic is charged~\cite{amazonprice,azureprice,googleprice}. Since the size of a cooperative request is small, each data center can initiate send requests to multiple destinations inexpensively and can receive the bulkier data packets free of charge.   We evaluate how fast we can recover using real world data in Section~\ref{sec:wide_area_results}.

\begin{comment}

\paragraph{In-Stream Recovery.} 

\john{If you agree with me that this should be the first priority, this logically goes before Cross-Stream}.  Finally, \sys{} also employs a traditional FEC-based recovery to provide a fast recovery option for random losses. This recovery method is only used when there are no cross-stream coded packets that can be used and an in-stream coded packet is readily available. \cody{Or maybe a tunable parameter can help choose FEC?}

For in-stream recovery, DC2 does not decode the in-stream packet itself. Similar to cooperative recovery, it parses the in-stream coded packet header \john{what meta-information is in this coded header?  we should specify.} and determines whether this packet is sufficient to enable recovery of a lost packet. If so, it sends the in-stream packet to the receiver for decoding.

Upon receipt, the receiver XORs the in-stream coded packet with other data packets received on the wide area Internet path to decode the lost packet(s), and delivers them to the application. %Algorithm~\ref{alg:in-stream-reco} shows the process by which DC2 decides to send an in-stream packet. 



%
% DC2 in-stream recovery
\begin{algorithm}[!t]
\scriptsize

\SetKwFunction{KwFnc}{start\_in\_recovery(lost\_flow\_id,lost\_seq\_num):}
\BlankLine
\KwIn{Flow id and sequence number of lost packet}
\BlankLine
\textit{// in-stream packets for lost packet }\\
\textbf{def} \texttt{\textbf{$in\_pkts[]$}}\\
\BlankLine
\BlankLine
\textit{// counting lost packets for a flow}\\
\textbf{def} \texttt{\textbf{$pkts\_lost$}}\\
\BlankLine
\KwFnc

\Indp
    \BlankLine 
    \textit{// for counting lost packets}\\
    \texttt{pkts\_lost $=$ 0}\\
    \texttt{lost\_entry $=$ (lost\_flow\_id,lost\_seq\_num)}\\
    
    \BlankLine 
    \textit{// fetch all in-stream packets}\\
    \texttt{in\_pkts[] $=$ get\_in\_pkts(lost\_entry)}\\                                                   
    \texttt{in\_count $=$ length(in\_pkts[])}\\
    \BlankLine
    \BlankLine
    \uIf{\texttt{in\_count $>$ 0} } {
        \texttt{in\_hdr $=$ get\_in\_hdr(in\_pkts[0])}\\
        \BlankLine
        \textit{// check lost status of all packets forming in-stream packet}\\
        \ForEach{\texttt{packed\_pkt in in\_hdr} } {
            \uIf{\texttt{marked\_as\_lost(packed\_pkt)}}{
                \texttt{pkts\_lost++} 
            } 
        } 
        \BlankLine
        \BlankLine
        \textit{// if we have enough in-stream packets, send them}\\
        \uIf{\texttt{in\_count $>=$ pkts\_lost } }{
            \texttt{dst\_addr $=$ get\_dst\_addr(lost\_entry)}\\
            \texttt{send\_fec\_pkt(dst\_addr,pkts\_lost,in\_pkts)}\\
            \Return{true} 
        }
    }
    \Return{false} 
 \caption{DC2 In-stream Recovery \cody{This is simple and not that interesting -- I propose we drop and just explain it in the text.}}
\label{alg:in-stream-reco}
\end{algorithm}

\end{comment}


\begin{comment}


% DC2 packet recovery design
\begin{algorithm}[!t]
\scriptsize

\SetKwFunction{KwFna}{perform\_loss\_recovery(flow\_id, seq\_num):}
\SetKwFunction{KwFnb}{start\_cross\_recovery(lost\_flow\_id,lost\_seq\_num):}
\SetKwFunction{KwFnc}{start\_in\_recovery(lost\_flow\_id,lost\_seq\_num):}

\BlankLine
\BlankLine
\textit{// Functions called after receiving a NACK}\\
\BlankLine
\KwIn {flow id and lost sequence number}
\BlankLine
\KwFna

\Indp
   \BlankLine
    \textit{// start recovery if it has not already started}\\
   \If{\texttt{!packet\_lost\_status(flow\_id, seq\_num)}} {
       \texttt{mark\_pkt\_lost(flow\_id, seq\_num)}
       \BlankLine
       \textit{// perform cooperative recovery first}\\
       \uIf{\texttt{!start\_cross\_recovery(flow\_id, seq\_num)}\\} {
          \texttt{start\_in\_recovery(flow\_id, seq\_num)}
       }
       \BlankLine
       \textit{// if both fail, relevant incoming coded packet will trigger recovery}\\
   }

\Indm
 \caption{ DC2 Packet Recovery Design}
\end{algorithm}
\end{comment}
%
%











\begin{comment}

\paragraph{Cooperative Recovery Workflow.}
Figure~\ref{fig:coop-recovery} shows an example of \sys{} with four receivers, R1 to R4, getting packets through direct Internet path. Receiver R4 experiences a burst of losses along the Internet path. In this case, in-stream coded packets will not be of any use: if they are sent along the direct path, they will likely also be lost, and if they are sent along the cloud path, the data packets needed to decode them will not be available. Cooperative recovery is the only option to recover such losses in a timely manner.

Due to this loss burst, R4 NACK timer will expire and it will send NACK packets to DC2 (Figure~\ref{fig:coop1}). 
If there are bursty losses, receiver will continue sending NACKs to DC2 until it starts receiving packets from the sender.
%Receivers send reports to DC2 to notify it of packets that have been successfully received. In cases of bursty losses or outages, timers will expire that force the receiver to send NACK packets to DC2 (Figure~\ref{fig:coop1}). This informs DC2 that there are potentially many losses occurring on the Internet path.

For every loss that DC2 recognizes through NACKs from the receiver, it determines if the packet can be recovered using 
a cross-stream coded packet or not.
In this example, cross-stream decoding is necessary and possible, as there are no NACKS from other receiver sharing the cross-stream coded packet.

DC2 then sends cooperative recovery requests to each of these other nearby receivers (Figure~\ref{fig:coop2}), who look in their caches of packets recently received by \sys{}, and send the requested packets back to DC2 in the form of cooperative recovery responses. DC2 waits for enough of these responses to perform recovery, potentially ignoring stragglers if enough cross-stream coded packets are present. It then decodes the lost packet(s) and transmits them to the lossy receiver (R4) (Figure~\ref{fig:coop3}).

Repeatedly applying this cooperative recovery algorithm not only enables \sys{} to recover an indefinite series of losses in most circumstances but
also makes the recovery process fast.



\subsection{Tuning Cloud Path Utilization}
\label{sec:tuning}
\fahad{unsure about this section. it's somewhat repetitive, but maybe useful in putting things together.}
\john{I think as is, it's on the redundant side.  If we had formulas or other quantification, it would deepen and unify this.}
\cody{Given lack of quantification, parts may fit better as philosophizing about, and highlighting the importance of, cross-stream coding in the Conclusion (and scrap the rest).}

We now distill the coding and loss recovery components of \sys{} into its broader contribution: what are the trade-offs involved in judiciously utilizing cloud paths for packet recovery? In doing so, we highlight the role and novelty of cross-stream coding in contributing to timely, robust, and inexpensive recovery.

\subsubsection{Coding Rate Tuning}

%We first consider how setting the coding rate parameters affects the temporal, spatial, and cost constraints of packet recovery.

%is non-trivial; knowing path characteristics such as the loss rate and distribution of the length of consecutive losses is helpful but not sufficient, since the application's loss tolerance, bit rate, and time budget are also relevant to the equation.

\paragraph{Temporal Constraints.} Generally, encoding over a greater number of data packets increases the time required for recovery, since most of those data packets need to be received in order for recovery to occur. This is especially true for in-stream coding, where all of the packets in question are arriving linearly as sent by a single application. However, part of the novelty of cross-stream coding is that it helps relieve this temporal constraint because recovery uses packets across streams that are flowing around the same time, so \sys{} does not need to wait through a stream of packets to do recovery. Additionally, the cross-stream coding rate can minimize the effect of stragglers in the cooperative recovery process, further reducing the time needed for recovery.
\john{focus this last sentence as a tradeoff maybe?}

\paragraph{Spatial Constraints.} For robustness of recovery, \sys{} can protect against random losses by setting the in-stream coding rate such that random loss episodes can be recovered up to the application's requirements -- the 99.9th percentile, for example. Here again, however, the cross-stream coding rate opens new interesting tradeoffs, since the rate can minimize the effects of correlated losses between Internet paths (or between Internet paths and the inter-DC path). For example, even if multiple flows experience outages or there are random losses on the inter-DC path, multiple cross-stream coded packets may be sufficient to recover all of the lost packets. In essence, cross-stream coding reduces the spatial complexity of packet recovery.  \john{I don't understand the use of spatial in this subsection -- not clarified.}

\paragraph{Cost Constraints.} To keep costs low, we want to minimize the number of bits transmitted from DC1 and DC2. DC1 always transmits all coded packets to DC2, but the recovery process then differs at DC2. For in-stream recovery, DC2 transmits to the receiver only the coded packets that will immediately help with recovery, while for cross-stream recovery DC2 transmits only cooperative recovery requests and the decoded packet(s) to the receiver. The cooperative recovery requests only specify what packet is being requested and are therefore small, and any decoded packets are roughly equivalent in size to the in-stream packets that would be sent between DC2 and the receiver. Therefore, cross-stream coding provides yet another benefit: \sys{} reaps the benefits of cross-stream recovery without significantly more overhead than in-stream recovery. \cody{Back of the envelope calculation?}  \john{I think so, otherwise this is a little too redundant and high-level, not enough deepening.}



%As \sys{} is intended for interactive applications where the average frame rate is 10-15 fps and the average frame size is 2-5 packets~\cite{} [\john{I don't think we've set something like this until now.  is this true in general?}]  it is best suited to send an in-stream packet for each frame. Hence, in-stream parameters $k_{in}$ and $n_{in}$ can be set to small, constant values. In our evaluations that simulate interactive applications, we set $k_{in} \gets 5$ and $n_{in} \gets 1$. We also use a minimum of two cross-stream coded packets to mitigate the effects of stragglers and protect against bursty losses and outages on the direct path. We vary number of data packets, $k_{cross}$, based on number of unique user streams utilizing \sys{}.


%The parameters $T_{in}$ and $T_{cross}$ are more closely tied to the time budgets of the participating flows; the longer \sys{} has to deliver packets, the longer it can wait to perform encoding across a full set of $k_*$ packets and therefore reduce the number of coded packets. In the case of cross-stream coding, $T_{cross}$ should be relative to the flow with the shortest time budget in the the batch.




%Table~\ref{table:1} shows the tunable parameters in \sys{}. Variables involved in coding ($k_*$, $n_*$, $T_*$) are set at DC1, variables involved in loss recovery ($\rho$, $\tau$) are set at DC2, and variables involved in loss detection ($\alpha$, $\sigma$) are set at the receiver.

%When deciding how to set these parameters, the \sys{} and application operators should consider: (1) how robust do you need recovery to be? (2) how fast do you need recovery to be? and (3) how much are you willing to pay? 


%% JB:  this is too basic to spell out.
%%
%%Clearly, the cheapest option is to not send %%any encoded packets ($n_{in} \gets 0$ and %%$n_{cross} \gets 0$) over the inter-DC path, %%but then \sys{} cannot provide any %%cloud-assisted recovery. Duplicating all data %%packets ($n_{in} \gets k_{in}$ and $n_{cross} %%\gets k_{cross}$) across the cloud path would %%provide extremely quick recovery (since no %%decoding would be necessary), but would be %%quite expensive.


%Note that \sys{} also has some latitude in selecting receivers that are close to DC2. Doing so helps ensure that cooperative recovery messages and recovered packets can be quickly sent between DC2 and receivers.

\subsubsection{Loss Recovery Tuning}
%As part of the loss detection algorithm, there are several parameters that can be tuned, including the threshold to start the optimized, proactive recovery at DC2 or the weight given to the inter-arrival time of new packets when dynamically setting a timeout at the receiver. These affect the sensitivity with which a loss is detected.
\cody{fold this into 3.3}

\end{comment}

%Since the cooperative recovery process involves many receivers sending their packets to the DC using the free ingress bandwidth, we proactively use this mode if any receiver reports a string of consecutive delayed packets (similar to a triple duplicate ACK in TCP), thus not waiting for the receiver to explicitly detect a loss.

\begin{comment}
% Uncomment \twocolumn below if the table needs to be split.
%\twocolumn
\bottomcaption{Tunable parameters in \sys{}.}
\renewcommand*{\arraystretch}{1.2}
\tablehead{\bfseries Parameter & \bfseries Description \\}
\begin{supertabular}{l p{5.5cm}}
\toprule
    $k_{in}$ & Batch size: max number of packets used to create in-stream coded packets at DC1. \\ \hline
    $n_{in}$ & Number of coded pac
    kets generated and sent alongside an in-stream coding batch. \\ \hline
    $T_{in}$ & Timeout to encode in-stream coded packets at DC1. \\ \hline
    $k_{cross}$ & Batch size: max number of packets used to create cross-stream coded packets at DC1. \\ \hline
    $n_{cross}$ & Number of coded packets generated and sent alongside a cross-stream coding batch. \\ \hline
    $T_{cross}$ & Timeout to encode cross-stream coded packets at DC1. \\ \hline
    $\rho$ & Preference of in-stream to cross-stream recovery at DC2. \cody{Maybe?} \\ \hline
    $\tau$ & Threshold to activate pro-active loss detection mode at DC2. \\ \hline
    $\alpha$ & Weight given to new interrarrival data when calculating the packet loss timeout at receivers, $T_{r}$. \\ \hline
    $\sigma$ & Tolerance for out-of-order packet arrival at receiver when detecting packet loss. \cody{Maybe?} \\ \hline
\bottomrule
\label{table:1}
\end{supertabular}

\end{comment}

\begin{comment}


We do not employ such scheme in \sys{} as conventional wisdom suggests that retransmitting packets on a wide area path will most likely have long recovery times, which results in retransmitted packet becoming obsolete for interactive application.

We now consider two potential schemes that could be used to detect losses in \sys{}, first one involves using nearby data center to detect losses, second involves receivers detecting losses and initiating recovery.

\paragraph{DC2 based detection:} In a data center based loss detection technique, receivers would send acknowledgments to DC2, which is their nearest data center (figure~\ref{}).
DC2 will have to implement two strategies to precisely detect losses, first is monitoring missing acknowledgments and second is maintaining timeouts for each packet per receiver. The first strategy requires initiating packet recovery for acknowledgments that are missing. Figure~\ref{} highlights this scenario, packet number 3 is lost and DC2 detects this loss by monitoring the ACKS received and initiates recovery for it. 
Now DC2 supplements this strategy by maintaining a timer for each pakcet per receiver, this helps in detecting bursty losses and also caters for lost ACKS from receiver. This timer mechanism is different from TCP, as DC2 is not the original sender, hence, it has no idea when packets are being transmitted by sender. Therefore, coming up with a precise timeout value is complex. This value requires DC2 to have prior knowledge of two variables, latency of sender -receiver-DC2 path and application packet sending rate. Furthermore this timer has to be set up for each packet per receiver, not only making it difficult to scale but also complex to implement. 

\paragraph{Receiver based detection:} In this technique, receivers are responsible
for detecting losses. Each receiver has a timeout value, that it takes as an input from the application. If a packet gets lost, receiver initiates recovery by contacting DC2. Figure~\ref{} shows this technique, upon timer expiry for packet number 3, receiver sends a NACK to DC2, which subsequently starts recovery. Using NACKs provides precise detection of lost packets and makes DC2 independent of application running on Internet path. In this technique, receivers can decide not only which packet to recover but also which interface to use for recovery. A smart receiver can detect losses on it primary interface and switch packet recovery to a secondary interface like mobile data to avoid further losses.

In \sys{}, we use receiver based detection technique as it gives more power to receivers and has a simple design.




\subsubsection{Loss Recovery}

Once the loss is detected, packet recovery is fairly simple. In \sys{}, recovery depends on the type of loss encountered by the receiver. If the loss is bursty, DC2 utilizes cooperative recovery couple with pro-active detection but if it is random, DC2 uses simple block based recovery. We now go into the details of these techniques.

\paragraph{Cooperative Recovery and Pro-active detection:} \sys{}'s primary loss recovery technique is cooperative recovery. This type of recovery is associated with cross-stream coded packets. Since, in this scheme, coded packet consists of multiple packets destined towards multiple destinations, in order to retrieve a single lost packet, DC2 sends requests to other destinations. Once DC2 receives all the required packets from other receivers, it generates the lost packet and sends it to original destination. This scheme makes use of current cloud pricing model, in which all incoming traffic is free. Since, cooperative request size is small, DC2 can afford to send it to multiple destinations and can receive actual data packets free of charge. 

Since \sys{} uses receiver based NACK recovery, we can make packet recovery faster by using pro-active loss detection mode. In this mode, if DC2 receives three consecutive NACKS from a receiver, it does not wait for future NACKs to start recovery. It marks that receiver and starts cooperative recovery for each relevant incoming coded packet.
DC2 switches back to normal recovery mode once it receives an ACK from 
receiver. This ACK indicates that receiver has started receiving packets from the sender again.

\paragraph{Simple Recovery:} This is the secondary loss recovery technique that \sys{} employs. It is similar to traditional forward error correction based recovery, hence, it is only useful if recovery from random losses is required. This method is only used when the following three conditions are met. First, detected packet loss pattern is random, second, there are no vertical cross-stream coded packets that can be used and finally if block in-stream coded packet can used to recover the lost packet. Since, in-stream block coding relies on other packets of same stream, it will add additional delays to loss recovery times, hence, we only use this method when absolutely required. 


\subsubsection{Loss Detection \& Recovery Algorithm}
\osama{step by step details along with algorithm for loss detection and recovery}

\subsubsection{Dealing with Stragglers and Losses}
While cooperative recovery helps in recovering from bursty losses and outages, there is an issue of stragglers and lost requests/responses that \sys{} must address. If any of the cooperative requests or responses get lost, we will not be able to perform packet recovery at all. Similarly, the recovery will not be timely, if one of the destinations is slow to respond to a cooperative request. To quantify these issues, we conduct a small experiment and determine the extent of this problem on PlanetLab paths.

In our experiment, we select a data center node in US and send cooperative requests to 10 nearby PlanetLab nodes. We send these requests every 10ms and log the responses back. We conduct this experiment for total of 24 hours with two separate 12 hour runs at different times. Figure~\ref{} shows the request response times for different numbers of receivers. IF we consider all receivers responses then 99\% of requests are never beyond a specific RTT (50ms), However, if we only wait for fastest n-1 response packets, we will get 99.9\% of responses in specified time limit and these recovery time do not change significantly for rest of fast receivers. 

\paragraph{Requirement:} Fast detection and recovery while incurring minimal cost. Highlight the differences with traditional approaches (e.g., TCP)

\paragraph{Our Approach.}
\begin{itemize} 
\item \textbf{Receiver is in-charge.} Receiver detects losses, can decide if any when to initiate recovery, can use any interface it wants. 

\item \textbf{Aggressive Use of the (Free) incoming DC bandwidth.} Cooperative recovery is pro-actively done after certain number of losses. Additional network cost is little because of incoming bandwidth is free as per today's pricing model. 

\end{itemize}


\paragraph{Protocol Details.}
Details including the steps performed by receiver, DC2, cooperative recovery nodes. 

\end{comment}

==> ReWAN-arxiv(1)/discussion.tex <==
\section{Discussion and Future Work}
\label{sec:discussion}

Our research opens up interesting future work, such as: 
\begin{comment}


\paragraph {Deployment model.} We believe a \sys{}-like service can potentially be deployed by the cloud infrastructure provider, an ISP, or a third-party service provider who pays the cloud operator only for the infrastructure usage. Users can explicitly opt into using \sys{} if they require a more reliable wide-area service -- for example, implemented as a paid service or added value proposition.
    %% JOHN:  I don't love the ads model -- or the service provider may use advertisements to generate revenue. 
    The deployment model may also have implications on the practical usage of \sys{} design. For example, an ISP or cloud provider with full control over its resources (e.g., using SDN~\cite{swan}) may prioritize the inter-DC coded traffic for even higher resilience and lower delay, leading to even higher recovery efficiency. 
    An ISP providing the service can also reduce sender overhead by duplicating the packets in the core as well.
 \end{comment}   
  \paragraph {Privacy and security considerations.} Duplicating traffic along cloud paths to be processed in data centers opens up the possibility of surveillance. At least one United States governmental program has collected traffic between data centers abroad~\cite{arnbak2014loopholes}. Future work could also study the privacy implications of network coding across multiple streams, and incorporate better privacy mechanisms in \sys{}.%to the coding and recovery design.%, since cooperative recovery involves asking nodes to transmit their data to a DC for decoding lost packets, leaking information about geographic location, stream rates, etc.
  %\fahad{we can possibly drop this if required. Also, not sure I understand privacy leak due to cooperative recovery  -- nodes only talk to DC2, not to each other}
  %\cody{I touched it up to be more general, but I would also be OK dropping this if needed.}
  
    \paragraph {Interface between \sys{} and the applications.} %The 
    \sys{}'s design involves various trade-offs involving performance and cost. We believe that ultimately the application (or the user) is in the best position to make suitable trade-off decisions, keeping in view its performance requirements as well as cost budget. Thus, exposing these trade-offs to the application through a suitable interface (e.g., through ChoiceNet~\cite{choicenet} or XIA~\cite{xiansdi}) is another promising research direction. 
  

%Can we compare cost of Via with cost of ReWAN? In other words, cost of selectively putting entire flow on relay path vs. cost of putting %coded packets on DC path for every flow. Or does the measurement/prediction aspect of Via make this comparison invalid? Such a discussion %could also go in the ``Cost'' or ``Related Work'' sections.

%A discussion of ReWAN being a component in a larger system (consisting of measurements, analytics, bandwidth provisioning, etc) could be %interesting, but perhaps out of scope.

%Might be a good place to discuss challenges or where \sys{} does not work (instead of Design).

%To improve cost of \sys{} even more, future work could code small packets with small packets and large packets with large packets to %reduce bandwidth usage on the inter-DC path.

==> ReWAN-arxiv(1)/evaluation.tex <==

\section{Evaluation}
\label{sec:evaluation}
We perform a multi-tiered evaluation with the goals of answering: 
 (1) How effectively does \sys{} recover packets within a time budget for wide-area paths (\S~\ref{subsec:pl-eval})?
 (2) How does \sys{} perform in the contexts of challenging application, transport, and network requirements (\S~\ref{subsec:skype-perf}, \ref{subsec:rewan-tcp-eval}, \ref{subsec:otherdeployment})?
 (3) How effectively does the \sys{} prototype scale to support the demands of many application streams, and what is the monetary and encoding cost of scaling up (\S~\ref{subsec:prototype-eval})?

  \begin{comment}
 We perform a multi-tiered evaluation with the goals of answering: 
 (1) How effectively does \sys{} recover packets within a time budget for wide-area paths (\S~\ref{subsec:pl-eval})?
 (2) How does \sys{} perform in the contexts of challenging application, transport, and network requirements (\S~\ref{subsec:skype-perf}, \ref{subsec:rewan-tcp-eval}, \ref{subsec:mobile-eval})?
 (3) How effectively does the \sys{} prototype scale to support the demands of many application streams, and what is the monetary and encoding cost of scaling up (\S~\ref{subsec:prototype-eval})?
  \end{comment}
 \begin{comment}
  (2) How effectively does \sys{} improve the user QoE of an interactive application (\S~\ref{subsec:skype-perf})? (3) How does \sys{} affect tail latency of tcp short flows?\osama{section ref and rethink question} (4) How can the \sys{} prototype scale to support the demands of many application streams (\S~\ref{subsec:prototype-eval})? \textcolor{blue}{(5) How do the challenges of mobile networks affect \sys{} (\S~\ref{subsec:mobile-eval})?}
 \end{comment}
 %
 %
  \begin{figure*}[!t]
\centering
  \subfigure[]{\includegraphics[width=1.37in]{graphs/recovery_rate_xinv_ccdf.pdf}\label{fig:rewan_recovery_overview}}
  %\hspace{0.2em}
  \subfigure[]{\includegraphics[width=1.37in]{graphs/loss_burst_overview_new.pdf}\label{fig:rewan_burst_overview}}
  \hspace{0.01em}
  \subfigure[]{\includegraphics[width=1.37in]{graphs/recovery_rate_fec_diff7.pdf}\label{fig:rewan_fec_diff}}
  \subfigure[]{\includegraphics[width=1.37in]{graphs/rtime_pl_new.pdf}\label{fig:rtime_rtt}}
  %\hspace{0.2em}
 \subfigure[]{\includegraphics[width=1.37in]{graphs/reco_diff_new3.pdf}\label{fig:reco_diff}}

  \caption{\sys{}'s performance on PlanetLab paths.(a) CCDF of successfully recovered packets. (b) Loss episode contribution to loss rate on paths with greater than 80\% recovery. (c) Percentage increase in \sys{} recovery rate vs FEC with 20\%, 40\%,and 100\% packet overhead on direct path (note x-axis). (d) Packet recovery times as ratio of direct path RTT. (e) Percentage increase in recovery rates using 2 cross coded packets per batch versus 1. }
\label{fig:rewan-all-metrics}
 \end{figure*}
 
 Our evaluation encompasses: 

\noindent\textbf{Wide-area Deployment and Evaluation.} We ran \sys{} on a public cloud for over a month and measured its effectiveness in recovering losses for 45 inter-continental PlanetLab paths (\S\ref{subsec:pl-eval}). Our results show that \sys{} is able to recover 78\% of the packet losses. Further, in  over 80\% of cases, the recovery time is less than half an RTT of the direct path between the sender and receiver. 
     
\noindent\textbf{Cross-Layer, Controlled Environment Evaluations.}
     We evaluate \sys{} with respect to user-level QoE metrics for Skype video conferencing (\S\ref{subsec:skype-perf}), flow completion time for short TCP flows (\S\ref{subsec:rewan-tcp-eval}), network QoS in a cellular setting (\S\ref{subsec:mobile-eval}), and other duplication strategies (\S\ref{subsec:deployment}). We find that in controlled environments, \sys{} can provide benefits up and down the stack, albeit with some environment-specific tuning to keep it cost-effective. 
    
\noindent\textbf{Scalability and Cost Evaluation.} We evaluate the scalability of our prototype (\S\ref{subsec:prototype-eval}) -- our results show that a single thread can handle 150 concurrent video calls and we can get linear speed-up as we increase the number of \sys{} threads. We also show
that the cost of supporting a large number of user streams is low compared to a full overlay solution.
 
     \begin{comment}
     comparatively evaluating \sys{} against Skype and its internal use of FEC. Our results show that \sys{}'s fast packet recovery translates into measurable QoE benefits under realistic network conditions -- it provides benefits similar to a complete overlay solution while consuming 86\% less inter-DC bandwidth.  
     
     \item \textbf{Tail Latency Reduction for TCP Short Flows}. We run \sys{} over TCP in an emulated environment with real world loss and latency values and show that \sys{} can reduce tail latency of short web flows by x\%. 
     
          \item \textcolor{blue}{\textbf{Effectiveness in Mobile Settings.} We evaluate how \sys{} performs with the additional constraints of a mobile network, and find that in most cases \sys{} can handle bandwidth and power concerns, but latency issues can reduce the cost-effectiveness of recovery.}
    \end{comment}
 
 
 
 
 %In essence, we evaluate \sys{} at the level of the application, network, and implementation.



%\cody{I also have results showing that Skype will accept recovered packets after a long time (even up to 200 ms), leaving plenty of time for recovery. This seems to be because as long as the latency is consistent, Skype tries to make it work. Therefore, there are hiccups when the recovery first begins (since it takes 10ms x 4 = ~40ms to recover a packet), but once that is done consistently for long outages, Skype adjusts and the video is fine. Not sure if this adds to what has already been said about Skype being amenable to \sys{}, so I have not included it for now.} 


\begin{comment}
\osama{nsdi18}
\begin{table}[!t]
\centering
\scriptsize
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccc}
\hline
Source & Destination & DC1 & DC2 & \begin{tabular}[c]{@{}c@{}}Num of \\ Active Paths\end{tabular} \\ \hline
\multirow{3}{*}{US East} & EU & Virginia & Netherlands & 8 \\
 & OC & Virginia & East Australia & 8 \\
 & Asia & Virginia & Japan & 3 \\ \hline
US West & EU & California & Netherlands & 8 \\ \hline
EU & OC & Netherlands & East Australia & 8 \\ \hline
OC & US West & East Australia & California & 8 \\ \hline
Asia & US West & Japan & California & 3 \\ \hline
\end{tabular}%
}
\caption{PlanetLab \& data center location and path information. }
\label{tab:planetlab_setup}
\end{table}

\end{comment}



\begin{comment}
\osama{old}
\begin{table*}[]
\centering
\scriptsize
\begin{tabular}{ccccccccc}
\hline
Source & Destination & DC1 & DC2 & \begin{tabular}[c]{@{}c@{}}Max \\ Samples\end{tabular} & \begin{tabular}[c]{@{}c@{}}Num of \\ Active Paths\end{tabular} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Max \\ Cross Coding \\ Block Size\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Coded Packets \\ / Block\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Cross Coding\\ DC1 Timeout\end{tabular}} \\ \hline
\multirow{3}{*}{US East} & EU & Virginia & Netherlands & 1 & 8 & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{\multirow{7}{*}{2}} & \multirow{7}{*}{70ms} \\
 & OC & Virginia & East Australia & 1 & 8 & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{} &  \\
 & Asia & Virginia & Japan & 1 & 3 & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{} &  \\ \cline{1-7}
US West & EU & California & Netherlands & 1 & 8 & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{} &  \\ \cline{1-7}
EU & OC & Netherlands & East Australia & 1 & 8 & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{} &  \\ \cline{1-7}
OC & US West & East Australia & California & 1 & 8 & \multicolumn{1}{c|}{6} & \multicolumn{1}{c|}{} &  \\ \cline{1-7}
Asia & US West & Japan & California & 1 & 3 & \multicolumn{1}{c|}{3} & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}%
\caption{PlanetLab \& data center location, path information, and parameters. }
\label{tab:planetlab_setup}
\end{table*}

\end{comment}


\begin{comment}


 \begin{figure*}[!t]
\centering
  \subfigure[]{\includegraphics[width=1.60in]{graphs/recovery_success_rate_new_ccdf.pdf}\label{fig:rewan_recovery_overview}}
  %\hspace{0.2em}
  \subfigure[]{\includegraphics[width=1.60in]{graphs/loss_burst_overview_new.pdf}\label{fig:rewan_burst_overview}}
  %\hspace{0.2em}
  \subfigure[]{\includegraphics[width=1.60in]{graphs/rtime_pl_new.pdf}\label{fig:rtime_rtt}}
  %\hspace{0.2em}
 \subfigure[]{\includegraphics[width=1.60in]{graphs/reco_diff_new2.pdf}\label{fig:reco_diff}}
  \caption{\sys{}'s performance on PlanetLab paths.}
\label{fig:rewan-all-metrics}
 \end{figure*}

\end{comment}
%(a) CCDF of recovered packets. (b) Loss episode contribution to loss rate on paths with greater than 80\% recovery. (c) Packet recovery times as ratio of direct path RTT. (d) Percentage increase in recovery rates using 2 cross coded packets per batch versus 1.}


 


\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[width=3.2in]{graphs/recovery_rate_fec_diff2.pdf}
 \caption{Difference in recovery rate. \sys{} vs FEC with 20\%, 40\%,and 100\% packet overhead on direct path}
 \label{fig:rewan_fec_diff}
\end{figure}
\end{comment}


%

\subsection{Wide-Area Deployment and Evaluation}
\label{subsec:pl-eval}

%add VM details as a footnote, perhaps but upto you?
\subsubsection{Setup} 
We have been running \sys{} as a service on five different DCs of Microsoft Azure~\cite{azure}, located in US, EU, Asia, and OC, for over a month. We use F1 type virtual machine, which is compute-optimized with 2.4 GHz single core and 2 GiB RAM. %\footnote{VM details at \url{http://tinyurl.com/vm-msft}}
We evaluate 45 PlanetLab wide area paths spanning four different continents\footnote{Exact path details can be found at \url{http://tinyurl.com/pl-paths}}.
%Table~\ref{tab:planetlab_setup} shows the exact location and number of paths between each DC location.

%We now evaluate \sys{}'s end-to-end network performance by deploying it on real world paths. We use PlanetLab~\cite{planetlab2} and Microsoft %Azure~\cite{azure} infrastructure to 
%test our prototype. In this experiment, our goals are to see (1) How much recovery does \sys{} provide? (2) What kind loss patterns affect \sys{} %recovery? (3) How fast can \sys{} recover packets? (4) How can we improve \sys{} recovery performance?

%We run \sys{} on approximately 45 PlanetLab wide area paths for one month and use Azure data centers near PlanetLab nodes as a cloud overlay. 

We run a simple constant bitrate application on the PlanetLab nodes. 
To observe long-term time-averaged behavior without overloading the paths, we use ON/OFF periods with Poisson OFF times and constant ON times. In each ON interval, we send packets for 5 minutes; we set the mean OFF time to be 55 minutes.
DC1 relays the start of each ON interval to senders using a separate control channel, thereby ensuring that 
senders are (loosely) synchronized. We use $r=2/6$ and $s=1/5$ as our coding parameters.
Given the high churn rate of PlanetLab nodes, the total samples collected from each path varies.  Typically, we recover 500-800 samples per path, which translates to 3-5 weeks of measurement collection.

%We use constant values for different \sys{} parameters to maintain a balance between faster recovery and bandwidth overhead.
%We mainly use cross-stream based packet recovery at DC2 to evaluate its full potential in real world loss patterns. We use
%$k = 6$, $r = 2/6$ as coding parameter i.e. we consider 6 different flows and generate 2 coded packets per 6 data packets.











\begin{comment}

  \begin{figure}[!t]
 \centering
 \includegraphics[scale=0.18]{graphs/dc1_epstat.png}
 \caption{25th percentile loss episode inter-arrival time for all paths. }
 \label{fig:rewan_dc_gap}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[scale=0.18]{graphs/loss_reco_overview.png}
\caption{Loss recovery rates for \sys{} across different regions. Error bars represent the 25th and 95th percentiles.}
\osama{change key name }
\label{fig:rewan_recovery_overview}
\end{figure}

\end{comment}


\begin{comment}

 \begin{figure*}[!t]
\centering

  \subfigure[Recovery time as ratio of direct path RTT]{\includegraphics[scale=0.16]{graphs/rtime_pl.png}\label{fig:rtime_rtt}}
  \hspace{2em}
  \subfigure[Recovery time value in miliseconds]{\includegraphics[scale=0.16]{graphs/rtime_pl_raw.png}\label{fig:rtime_raw}}
  \hspace{2em}
  \subfigure[RTT betweenDC2 and receivers in different regions]{\includegraphics[scale=0.16]{graphs/receiver_dc2_rtt.png}\label{fig:rec_dc2_rtt}}
   \hspace{2em}
  \caption{\sys{} recovers lost packets within time budget }
  \label{fig:rewan_recovery_time}
 \end{figure*}


 \begin{figure*}[!t]
\centering

  \subfigure[Loss episode contribution to loss rate on paths with greater than 80\% recovery.]{\includegraphics[scale=0.16]{graphs/loss_burst_overview.png}\label{fig:rewan_burst_overview}}
  \hspace{2em}
  \subfigure[Loss episode contribution to loss rate on node-dc paths with less than 80\% recovery.]{\includegraphics[scale=0.16]{graphs/bdet_dc1.png}\label{fig:rewan_dc1_burst}}
  \hspace{2em}
  \caption{\sys{} Loss patterns on different paths.Random episodes are of length 1, Multi has 2-14 burst length, and outages have >15 burst length.}
  \label{fig:rewan_patterns}
 \end{figure*}
 
\end{comment}




%\osama{need to add straw man solution 1) fec only analysis with fixed block size and 1,2,4 coded packets (compare recovery with cost as well). 2) highlight actual recovery time and receiver to DC2 latency more 3) if time allows compare with maelstorm like scheme 4) for skype: add frame comparison picture to quantify losses. 5) highlight where we compare with straw man/existing solution e.g. skype built-in fec, tcp basic loss recovery, planetlab fec only}


\subsubsection{Results}
\label{sec:wide_area_results}
Our wide-area evaluation makes five key findings, summarized below, and visually in 
Figure~\ref{fig:rewan-all-metrics}.% and~\ref{fig:rewan-s-and-t}.

\paragraph{Most losses happen on wide-area links and \sys{} is able to recover them.} 
\sys{} is able to recover 78\% of all packets that are lost on the PlanetLab paths. Loss rates on these paths are relatively high: up to 0.9\% loss, with 40\% of paths having a loss rate greater than 0.1\%.  Overall, we lose 0.02\% packets in our experiment and we consider any packet that takes longer than one RTT to recover as a lost packet. As we discuss later, most of the packets that \sys{} is unable to recover are lost on the access paths. If we ignore those losses, \sys{}'s packet recovery goes up significantly. % \john{Why do we emphasize this 98\% number -- it seems artificial.}
%
Figure~\ref{fig:rewan_recovery_overview} elaborates on the above results -- it shows a CCDF of the fraction of successfully recovered packets (i.e., those lost packets that are recovered within one RTT) for all PlanetLab paths. Most paths experience high recovery (low unrecovered packet rate) -- overall, 82\% of paths successfully recover more than 80\% of lost packets.
%\osama{todo: analyze without perfect network i.e. fec is also lost, how to present better e.g. fec overhead instead of num of fec packets }

%Figure~\ref{fig:rewan_fec_diff} also shows the result of using traditional FEC scheme instead of \sys{}. We perform a what-if analysis with $s=\frac{1}{5}$ and $s=\frac{2}{5}$. We also assume perfect network conditions for these coded packets i.e. they \emph{always} reach the receiver even in the case of bursty losses or outages. We observe that with 1 FEC packet, only 4\% of paths have a recovery rate of greater than 80\%, whereas with 2 FEC packets, the number of paths %with same recovery rate 
%increase to 40\%. While \sys{} has higher (60\%) overhead on source-DC1 path, cross-stream coding ensures that 82\% of paths achieve greater than 80\% recovery rates.
%}
%we generate 1-2 coded packets and assume perfect network conditions
%%
%%JB out: (equivalently, 18\% of paths fail to recover at least 20\% of losses). 

\begin{comment}
 \begin{figure}[!t]
 \centering
 \includegraphics[scale=0.18]{graphs/loss_burst_overview.png}
 \caption{Loss episode contribution to loss rate on paths with greater than 80\% recovery. Random episodes are of length 1, Multi has 2-14 burst length, and outages have >15 burst length.}
 \label{fig:rewan_burst_overview}
\end{figure}
\end{comment}
\paragraph{\sys{}'s coding is able to handle a wide range of loss patterns.} We next zoom into the loss patterns to understand what types of losses are being recovered by \sys{}. Figure~\ref{fig:rewan_burst_overview} shows a CDF of loss episode patterns observed on PlanetLab paths that have greater than 80\% packet recovery (82\% of total paths). We look at the burst length of the loss episode and classify them as Random (single packet loss), Multi-Packet (2-14 packets), and Outage ($>$14 packets). We observe all three types of loss patterns on the chosen paths. While random and multi-packet bursts contribute more towards the loss rate, outages are not uncommon on these paths. Our data shows that 45\% of paths see outages that last from 1 to 3 seconds. Our recovery rates show that \sys{} is able to handle multiple types of burst lengths, quickly.
%% jb - duplicate, comes in one second...
%-- as we show later this recovery is also within a short time budget. 

%  \begin{figure}[!t]
% \centering
% \includegraphics[scale=0.18]{graphs/bdet_dc1.png}
% \caption{Loss episode contribution to loss rate on access paths.}
% \label{fig:rewan_dc_burst}
%\end{figure}
\paragraph{Most access losses can be recovered using existing techniques.} 
While access losses (between source-DC1 and DC2-receiver) are not the main focus of \sys{}, we look at their loss characteristics to see whether well-known techniques can be used to recover such losses.  Our results show that around 98\% of such losses occur on source-DC1 paths and that a significant fraction, 90\%, of loss bursts are single packet losses and can be recovered using simple retransmissions (ARQ) or other simple redundancy based techniques (e.g.,~\cite{gentleaggression}) at the edges (i.e., between the end-points and the DCs).  In future, we plan to augment \sys{} to incorporate this observation.

%\textcolor{red}{
\paragraph{\sys{} vs. On-Path FEC schemes.}
To compare \sys{} with traditional, on-path FEC packet recovery schemes, we perform a what-if analysis on the probes sent on the direct PlanetLab paths.
Our goal is to compare \sys{} with sending different number of FEC packets on the direct path. 
We divide the probes into 5 packet bursts and consider the next burst as the FEC packets. 
We then compute recovery success rates for 20\% ($s=\frac{1}{5}$), 40\% ($s=\frac{2}{5}$), and 100\% ($s=\frac{5}{5}$) FEC overhead. We also assume that, for \sys{}, access losses can be recovered using existing ARQ-based techniques. 

Figure~\ref{fig:rewan_fec_diff} shows the percentage increase in recovery rates for all the paths using \sys{}, compared to different levels of FEC. We observe that, even at 100\% overhead (full duplication), 90\% of the paths had at least one loss episode
that could have been recovered using \sys{} but not with on-path, 100\% FEC overhead. 
Further, 10\% of the paths observe more than 160\% improvement in recovery rates with \sys{} compared
to full, on-path duplication. These are paths that experience long burst of losses or outages that cannot be recovered using FEC on the direct path.  For 20\% overhead scheme, 100\% increase in recovery rate is seen by 70\% of the paths. This result shows that there exist paths for which \sys{}'s cross-stream coding is more effective in recovering from outages and bursty losses compared to traditional, on-path FEC based schemes.
%}

%30\% of that paths see at least 10\% improvement in recovery rates. Lower overhead schemes perform much worse than \sys{} as well. We observe that, for lower overhead schemes, more than 85\% of paths see at least 34\% improvement in recovery. 
%This confirms that \sys{}'s cross-stream coding helps in recovering from bursty losses and outages when fully duplicating on Internet path fails.
%Figure~\ref{fig:rewan_fec_diff} shows the difference in recovery rates compared to \sys{} for these schemes. For 40\% (resp. 20\%) overhead scheme, \sys{} has better recovery rates in 75\% (resp. 90\%) of all paths. Even if we assume 100\% overhead, i.e., full duplication on the direct path, \sys{} still provides better recovery in 50\% of paths, without adding congestion in the core. We also observe that \sys{}'s lower or equivalent performance on the other 50\% of paths is due primary to losses in the access paths. We outline how to deal with access losses next.
%}

%In our next release, we will augment \sys{} to incorporate this observation.

%\osama{compute x percentile distance between loss burst for all paths, plot a cdf for that showing most bursts have enough gap in them for applying %retransmission schemes.}.
\begin{comment}
  \begin{figure}[!t]
 \centering
 \includegraphics[scale=0.18]{graphs/rtime_pl.png}
 \caption{Packet recovery times as ratio of direct path RTT. Most packets are recovered within 0.5 RTT}
 \label{fig:rtime_rtt}
\end{figure}
\end{comment}

\paragraph{\sys{}'s loss recovery is usually fast.}  We next look at packet recovery time using \sys{}, which  Figure~\ref{fig:rtime_rtt} depicts for paths in different regions. We show our recovery times as a ratio of direct public Internet path RTT between the source and destination. 
We note that 95\% of packets are recovered within 0.5 $\times$ RTT. As expected, we observe faster recovery for paths with higher absolute latency on the direct public Internet path. For example, on low RTT paths between the US and EU (110-130 ms), we see higher recovery times as a proportion of RTT, but in terms of absolute latency, 90\% of packets are retrieved within 75 ms. We also observe that receiver-DC2 RTTs on these paths vary significantly. For example, the RTT between receivers in the EU and their nearest data center varies from 16-70 ms ($\mu$ = 28 ms).
%(0.12 $\times$ RTT) 
%(0.5 $\times$ RTT) with an average of 28ms (0.2 $\times$ RTT). 
However, as cloud providers continue to strive towards reducing their latency to end-users~\cite{mappinggoogle}, we expect \sys{} recovery times to continue to improve over time.

Finally, we observe two systematic reasons contributing to the tail in the recovery time (Figure~\ref{fig:rtime_rtt}): delay in detecting and recovering a loss (e.g., due to delayed NACKs) and delay in arrival of coded packets at DC2. Overall, the percentage of recovered packets that fall outside of a reasonable time budget value is low and only accounts for roughly 1\% of the recovered packets.

\paragraph{Recovery time is improved due to straggler protection.}
%\osama{update text for removed figure}
Last, we show the benefit of using extra cross-stream coded packets to provide protection against stragglers during cooperative recovery. Figure~\ref{fig:reco_diff} %and Figure~\ref{fig:rtime_diff} respectively 
shows the performance gains using two cross-stream coded packets per batch, as opposed to one. With adequate protection of two packets per batch, 60\% of paths see greater than 10\% improvement in recovery rates (Figure~\ref{fig:reco_diff}). %Similarly, Figure~\ref{fig:rtime_diff} shows 
We also observe that the recovery times decrease by at least 50 ms for 70\% of the recovered packets (not shown) -- in some instances, the difference is some stragglers that take several seconds.%, indicated by the long tail of the graph (note the log scale). 
This further justifies our choice of default parameter values for PlanetLab paths.

%
%(~\cite{}), these latencies will decrease in the future.
%Similarly, the RTT between EU and OC paths is high (300-360ms), so recovery times are low not only as a ratio of RTT but in terms of actual value as well. The RTT between OC nodes and their nearest data center varies from 14ms to 45ms with an average of 33ms.
%
%Approximately 71\% of late recovered packets were due to late responses from receivers and 29\% of late recovered packets were due to late arrival of %data packets at DC1.
%
%Approximately 71\% of late recovered packets were due to late responses from receivers. Since our clocks are not synchronized, we cannot be sure whether delay occurred on the forward or reverse DC2-receiver path. However, we do observe that PlanetLab nodes respond immediately (within 1ms) to requests and cloud nodes perform recovery as soon as they receive coded packets. Overall, 53\% of paths were affected due to this type of late recovery. 
%
%Around 29\% of late recovered packets were due to late arrival of coded packets at DC2. After analyzing coded packet generation times at DC1, we observe that these late arrivals were due to slow processing of incoming packets at DC1. Since we are using a low end virtual machine with limited bandwidth at DC1, a small percentage of packets were processed late due to high load. We believe these delays can be reduced by using a high end machine with high bandwidth. Overall, only 40\% of paths suffered from this issue. 
%
%
\begin{comment}
 \begin{figure}[!t]
\centering

  \subfigure[]{\includegraphics[scale=0.12]{graphs/reco_diff.png}\label{fig:reco_diff}}
 
  \subfigure[]{\includegraphics[scale=0.12]{graphs/rtime_diff.png}\label{fig:rtime_diff}}
  \caption{}
  \label{fig:rewan_straggler}
 \end{figure}
 
\end{comment}
%
%
%
%
%
\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.18]{graphs/reco_diff.png}
 \caption{Percentage increase in recovery rates using 2 cross coded packets per batch versus 1.}
 \label{fig:reco_diff}
\end{figure}
%
%
\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.18]{graphs/rtime_diff.png}
 \caption{Difference in packet recovery times when 2 cross-stream coded packets per batch versus 1.}
 \label{fig:rtime_diff}
\end{figure}
\end{comment}
\subsection{Skype Performance with \sys{}}
\label{subsec:skype-perf}

We run \sys{} under Skype's video conferencing service to measure its effect on an interactive application.\footnote{Skype is transitioning some of its services from peer-to-peer to a cloud architecture, but that shift is incomplete as of submission time~\cite{skypecloud}; therefore, Skype's traditional peer-to-peer video conferencing architecture is used in this evaluation.}  We focus on the performance of Skype in wide-area settings where outages occur (similar to ones described earlier in our wide-area evaluation). To do so, we leverage the cloud path to run the video conference in three experiments. First, we examine how the video quality degrades during an outage along a public Internet path used by Skype. We then duplicate \textit{all} Skype packets over a cloud path to show that such a path can indeed make up for lost packets during outages. Finally, we use \sys{} to selectively transmit coded packets over the cloud path and perform recovery at the receiver.
%, showing that \sys{} attains nearly identical performance benefits at a fraction of the cost.

%We also replay packet traces of wide area paths that we previously measured to test Skype's performance during packet outages.
% using a Linux traffic control facility, NetEm~\cite{netem}.

%When Skype transmits a packet, we intercept it using the \sys{} prototype and duplicate it on the cloud path.

\subsubsection{Testbed and Measurement Procedure} We use a similar testbed to that used by Zhang et al.~\cite{zhang2012profiling}, in which clients communicate using Skype's video conferencing service. We connect clients running Skype for Linux 4.3 in a LAN, and emulate wide area path characteristics such as latency, packet loss rate, and jitter.

We use Skype's screen sharing mode to transmit a pre-recorded video that closely represents the normal motions of human interaction during a video conference. We then compare the quality of each received video against the reference video by converting all videos to raw (uncompressed) format, and compute objective QoE scores on a frame-by-frame basis using VQMT~\cite{vqmt}. Although objective video quality metrics are not as reliable as subjective metrics given by users (such as Mean Opinion Score), they are sufficient to approximate the quality of the video on a frame-by-frame basis. We show the scores of each frame in a CDF to approximate the quality of each video in aggregate.
% we use a well-known news anchor video sequence, ``Akiyo,'' from the ITU's Joint Video Team repository. On the receiving end, we perform a fixed-size screen capture and sync the captured video with a reference video.
%These scores include the peak signal-to-noise ratio (PSNR), structural similarity, and multi-scale structural similarity, but since all of the objective metrics we used show similar results, we only display the PSNR scores in our analysis. 




\subsubsection{Results}


\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.16]{graphs/caspr_skype_eval.png}
 \caption{PSNR scores of a video conference sent over different network conditions and paths.}
 \label{fig:rewan_skype_eval}
\end{figure}
\end{comment}

\begin{comment}


%keepaspectratio
 \begin{figure}[!t]
%\centering
  %\hspace{-1em}
  \subfigure[]{\includegraphics[width=2.05in]{graphs/skype_new2_cb.pdf}\label{fig:rewan_skype_eval}}
  \hspace{-0.60em}
  \subfigure[]{\includegraphics[width=1.05in]{graphs/rewan_tcp_new3.pdf}\label{fig:rewan_tcp}}
  \caption{a) PSNR scores of a set of video conferences,  b) Tail of TCP flow completion times (note y-axis scale).}
  \label{fig:rewan-s-and-t}
 \end{figure}

\end{comment}


%\paragraph{Skype is flexible to packet recovery.} We first test whether Skype is amenable to a packet recovery service running beneath it. We start a video conference between two clients and send packets along both the Internet path and overlay path. During the call, we impose 100\% loss on the Internet path. Therefore, packets arrive only from the overlay path. We increase the one-way latency of the overlay path by 10 ms per experiment, looking for video quality degradation or a network change in Skype. We tested up to 200 ms -- well past the one-way latency of 150 ms traditionally considered acceptable for video conferencing (cite) -- and found that Skype video quality did not degrade in terms of PSNR score, since the one-way latency was consistent. 

\paragraph{Duplication using the cloud overlay enables higher QoE.} Figure~\ref{fig:rewan_skype_eval} shows the video quality results as we vary the network conditions and paths used. When a 30 second outage occurs along the Internet path, Skype's built-in FEC mechanism is insufficient to maintain an acceptable level of QoE. The video quality degrades with pixelation and frozen video, and the number of frames with poor PSNR scores significantly increases. Due to the high availability of the cloud path, when we duplicate all Skype data across the cloud path during the 30-second Internet path outage, virtually all packets reach the destination, preserving the video quality (similar to an Internet path with a 0\% loss rate). This shows that Skype is amenable to a packet recovery service running in tandem with it to correct losses on its direct public Internet path.

\paragraph{\sys{} achieves similar QoE compared to cloud duplication.} When running Skype over \sys{}, we disable in-stream coding on the cloud path ($s = 0$), since Skype uses its own FEC techniques on the Internet path to recover lost packets~\cite{chitchat}. To use cross-stream coding, we inject three \textasciitilde200 Kbps background UDP flows whose packets are coded with Skype packets at DC1 at a rate of $r = 1/4$, with $k = 4$. Figure~\ref{fig:rewan_skype_eval} shows that \sys{} achieves a similar level of QoE compared to duplicating across the cloud path. %Figure~\ref{fig:frames} shows the difference between a frame captured while Skype is running over \sys{} compared to the same frame captured during packet loss along the Internet path.

\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.32]{figures/frame_closeup.png}
 \caption{A comparison of the same frames during a Skype call running over \sys{} (left) and using an Internet path only (right) during a bursty loss of packets.}
 \label{fig:frames}
\end{figure}
\end{comment}

\paragraph{\sys{} uses significantly less bandwidth than cloud duplication.} Because Skype uses its own FEC, we only need to utilize cross-stream coding and recovery, reducing the amount of inter-DC bandwidth used. We also observed the inter-arrival time of packets during Skype calls, and tuned \sys{} accordingly by setting the NACK timeout value to 25 ms. This reduces the number of false positive NACKs that trigger unnecessary cooperative recovery. By taking advantage of this application-specific knowledge, \sys{} achieves similar QoE scores as full cloud duplication but uses much less bandwidth: in our experiments, \sys{} sent just 13.4\% as many packets and 13.6\% as many bytes as did the full utilization of the cloud overlay.


%the full cloud overlay sent an average of 19,742 packets and 12,156,088 bytes during the two minute video conference, while \sys{} sent %just 2,655 packets consisting of 1,661,197 bytes. Therefore,

%\john{This section is really solid and well-written.  I'm curious as to more details of how cross-stream was performed though:  we do not describe how many concurrent connections were routed along DC-DC paths, or what their characteristics were.  just saying UDP cross-traffic is not enough.}
%keepaspectratio

 \begin{figure}[!t]
%\centering
  %\hspace{-1em}
  \subfigure[]{\includegraphics[width=2.05in]{graphs/skype_new2_cb.pdf}\label{fig:rewan_skype_eval}}
  \hspace{-0.60em}
  \subfigure[]{\includegraphics[width=1.05in]{graphs/rewan_tcp_new3.pdf}\label{fig:rewan_tcp}}
  \caption{a) PSNR scores of a set of video conferences,  b) Tail of TCP flow completion times (note y-axis scale).}
  \label{fig:rewan-s-and-t}
 \end{figure}
%graphs/rewan_tcp_new3.pdf
\subsection{TCP Performance with \sys{}}
\label{subsec:rewan-tcp-eval}
We now evaluate the performance of TCP if it is used over \sys{}. Our goal is to understand how the additional reliability provided by \sys{} interacts with TCP's own reliability and congestion control mechanisms, and whether it can provide any additional benefits. We focus on TCP short flows as they are latency sensitive and do not require high throughput.

%We also evaluate overhead of \sys{}'s loss detection mechanism in terms of spurious recoveries performed by receiver.
\paragraph{Experimental Setup.} Our experimental setup is inspired by a similar experiment conducted by Google to evaluate different loss mitigation techniques for their web transfers~\cite{gentleaggression}. Using Emulab, we emulate the same topology and loss model as used in the Google study:  we consider a 200 ms RTT between end hosts and loss probabilities of 0.01 for losing the first packet in a burst and 0.5 for each subsequent loss. Given our focus on understanding TCP's interaction with \sys{}, we consider a single client-server scenario, in which a client sends a 12B request and receives a 50 KB response from the server. The RTT between server/client-DC paths is 30 ms with an RTT of 200 ms on the DC1-DC2 path. We make 10K requests each for TCP and TCP over \sys{}. 

%We perform this experiment on Emulab and we do not introduce any loss on overlay path (Server-DC1-DC2-Client). W

%Given our focus on understanding TCP's interaction with \sys{}, we disable coding at DC1 and directly send packets to DC2, where they %are stored and recovered only in case of a NACK. Although our results do not fully add latency of encoding and recovery process, we %believe that, in context of flow completion times, this delay will not be significant.% enough to change any results. 




%For this experiment, \sys{} is only running from server to client i.e. server acts as a \sys{} sender and client as a \sys{} receiver
 
\begin{comment}


\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.15]{graphs/rewan-tcp.png}
 \caption{TCP performance with and without \sys{}}
 \osama{placeholder}
 \label{fig:rewan_tcp}
\end{figure}
\end{comment}

\paragraph{\sys{} reduces tail latency for lossy short flows.}
Figure~\ref{fig:rewan_tcp} shows TCP's flow completion times with and without \sys{}. We observe that TCP suffers from long latency tail that goes up to 9 seconds, whereas \sys{} reduces the tail significantly. Our analysis shows that TCP is able to recover from most of the losses (using SACK), but there are some losses which are problematic for TCP, and hence cause the long tail. Such losses typically occur at the start of the connection, e.g., SYN-ACK(s), or at the very end. Such losses cause 
TCP to timeout, and successive losses mean that these timeout values could become huge, resulting in the long tail for TCP. 
\sys{} is able to reduce flow completion times by quickly recovering these losses. As soon as a packet is recovered by \sys{}, our TCP client sends an ACK to the server, effectively hiding the loss, and avoiding TCP timeouts. 

%This delayed SACK makes sure that TCP does not go into congestion avoidance mode by assuming packet loss. Therefore, by providing added %reliability at beginning and end of flow, \sys{} is able to reduce flow completion times.

%We do observer that losses experienced in the middle of the connection are easily handled by TCP, as it has capacity to send packets in %the subsequent windows. 

%Losses at the beginning of the connection mean that SYN-ACK(s) from the server were lost and the client backs off before making another attempt. Similarly losses at the end cause RTO to expire at the server side, forcing TCP to exponentially back off. Both these scenarios cause TCP to go in to congestion avoidance mode, hence, affecting flow completion times.

%which causes flow completion times to shoot up in seconds and ultimately affect user experience. 
%In this experiment, TCP uses three round trips to fully send data, it sends 10$\times$MSS packets in first window, 20$\times$MSS packets in second window and 7$\times$MSS packets in the third window.
%\paragraph{\sys{}'s fast recovery masks losses from TCP.} 

\paragraph{Two State Markov Model Reduces Overhead.} Note that TCP sender's control loop is quite different than the open loop CBR senders we have considered in our prior experiments. Our analysis also shows that our simple two state Markov model is able to adjust to TCP sender's control loop, specifically slow start, by using a smaller timeout in the middle of the window, and using a larger timeout across windows and subsequent transfers. Compared to maintaining a single timeout value, the two state approach results in 5x fewer NACKs sent to DC2. 

%\osama{overhead of \sys{} timer 10\% without optimization, 2.6\% with current setup (no sync b/w dc2 and receiver). Not sure about %overhead of proposed method}


%Meanwhile a server might have already retransmitted the recovered packet due to SACKs from the client, we are able to maintain optimal flow completion times by recovering the packet early. 

%Although these results are in a controlled environment, we can see that \sys{} can provide benefits for TCP short flows by reducing tail latency. However, for a long running TCP connection, \sys{} fast recovery will not provide similar benefits as flow completion times are already in the order of seconds.


%While server might have already retransmitted the packet, this SACK makes sure that server doesn't go into congestion avoidance mode. Similary, if a SYN-ACK is recovered after a small delay, both client \& server can assume attribute delay to the network. 
%reduce the long tail experienced by short flows on web. 

\subsection{Prototype Scalability and Cost}
\label{subsec:prototype-eval}

%\subsubsection{Goal and Setup}

\noindent\textbf{Scalability.} We benchmark the performance of our prototype in terms of the number of encoded packets at DC1, since it is the most computationally expensive component of \sys{}. Our goal is to measure how efficiently \sys{} can process and encode packets as the system scales to a large number of concurrent streams. %We also quantify bandwidth and compute costs of our prototype using current cloud pricing model.
%Algorithm~\ref{alg:dc1} is the most computationally expensive component of \sys{}, since every data packet in a stream is encoded into one or more coded packets. The DC2 node also performs a computationally-intensive decoding task, but the expense of decoding is comparable to that of encoding, and the number of invocations of the decoding algorithm is significantly lower as it is only called when packet loss is detected. Therefore, we consider DC1 to be the most likely potential bottleneck and focus our benchmarking tests there.
For each flow, \sys{} is configured to generate a single coded packet per every five data packets. We use Dell Poweredge R430 servers on Emulab, and each server is equipped with two 2.4 GHz 8-core processors with two threads each, for a total of 32 hardware threads.%, and each with an
%JB: very weird:  at least one -- when do we use multiple NICs ?
%Intel X710 10Gb Ethernet NIC. 

\begin{figure}[!t]
 \centering
 \includegraphics[width=3.2in]{graphs/scale_new.pdf}
 \caption{Throughput of the \sys{} prototype scales linearly with the number of encoding threads. Eight threads can handle up to 500Kpps.}
 \label{fig:proto_eval}
 % Cody -- done. \osama{this figure can also be reduced as well.}
\end{figure}

We first determine the maximum throughput achievable at DC1 in packets per second. Measuring packets (instead of bits) is the appropriate measurement granularity because the encoder operates over entire packets. 
%Using a single encoding thread at DC1, 
We find that a single encoding thread can handle around 65 Kpps. For context, assuming an average packet size of 512 bytes, 65 Kpps is enough for performing one-way processing for \textasciitilde150 simultaneous HD Skype video calls~\cite{skype_bw}. At this rate, the bottleneck is the generation of coded packets from data packets.
% -- our results show that packet size does not significantly affect the encoding and decoding time for realistic packet sizes

%We then consider how parallelism in encoding can relieve this bottleneck and increase throughput. To do so,
We then increase the number of DC1 encoding threads as we increase the number of senders, and load balance the streams to the different encoding threads. We rate limit each sender to 65 Kpps -- the empirical maximum rate that can be processed by a single (sender, encoder) pair. Figure~\ref{fig:proto_eval} shows that the processing power of \sys{} scales linearly with the number of encoding threads: up to \textasciitilde500 Kpps with eight encoding threads. %This trend would likely continue up to the limits of the CPU and NIC of the node.
This shows that \sys{} is amenable to parallelism and can be deployed in software to handle a large number of users. 

%commenting it out for now

\noindent\textbf{Deployment Cost.} For estimating \sys{} deployment cost, we do a %by doing
back-of-the-envelope calculation that compares \sys{} with a solution that fully uses the cloud. Based on the bandwidth requirement of Skype, a single user will send 0.675 GB of data per hour. Since a single \sys{} thread can handle 150 Skype calls, a data center node in an overlay will receive and forward $\sim$101 GB of data per hour, for 150 parallel application sessions. For a 2-node overlay node, based on today's cloud pricing~\cite{azureprice}, this would cost a minimum of \$17.60/hour for bandwidth and \$0.13/hour for single thread general purpose compute usage. However, for \sys{} using a coding rate of $r=1/16$, the \emph{maximum} cost of bandwidth for 150 calls will only be \$1.10/hour, which is 16x less than the cost of a full overlay. In this calculation, we are assuming that every coded packet will be used to recover a lost packet, which is an upper-bound on the overhead of \sys{} --  in practice, the outgoing bandwidth from DC2 will only be used in case of a packet loss.  

%Also, changing the coding rate to $1/8$ or $1/16$ significantly reduces the cost to \$2.20 and \$1.10 respectively. 



\noindent\textbf{Coding Overhead.} Due to limited availability of PlanetLab nodes, our wide area experiments considered a small number of concurrent user streams for encoding (typically $k=6$). 
We have also conducted experiments in Emulab to validate the feasibility of encoding over larger number of concurrent streams, which can further reduce the overhead of coded packets. 
Our controlled experiment, which used loss rates from Google's study (as in our TCP experiment), shows that for 20 concurrent streams and 2 cross stream coded packets (i.e., $r=2/20$), 
we can recover more than 92\% of the lost packets, for a coding overhead of only 10\%. 

\subsection{Other Deployment Scenarios}
\label{subsec:otherdeployment}
%\textcolor{red}{
Our focus so far has been on scenarios with well connected endpoints. 
We now explore the potential use of \sys{}
in challenging scenarios, such as cellular access networks or 
when full duplication at source is infeasible. 

\subsubsection{Mobile Networks with \sys{}}
\label{subsec:mobile-eval}
The design of \sys{} makes assumptions that can be challenged in mobile networks, since mobile settings have different bandwidth, power, and latency characteristics.

\paragraph{Duplicating traffic can be feasible.} 
The bandwidth provided to cellular devices can vary greatly~\cite{sprout2013} -- our survey of major US carriers shows users can typically expect 2-5 Mbps uplink bandwidth. Therefore, we consider whether the most bandwidth intensive part of \sys{} -- the duplication of traffic to the cloud path at the sender -- works within the link rates of mobile networks.

We modified our Skype testbed (\S\ref{subsec:skype-perf}) to tether the sending host to a mobile device connected to an LTE network, and observed that the overall bandwidth required by \sys{} to duplicate a Skype video stream (1.5 Mbps) is well within the uplink bandwidth %provided to us by T-Mobile
, which we measured to be $\sim$5.0 Mbps. However, the recommended bandwidth for HD video calls in Skype is 1.5 Mbps~\cite{skype_bw}, so duplicating that traffic to over 3.0 Mbps could reach the capacity of uplinks in some networks. We also tested how \sys{} affects other ongoing transfers on the device, and found that the transfer time for 5 MB files over WhatsApp is not affected by \sys{} running simultaneously.
%T-Mobile's

For data-intensive uses, \sys{} may need to more selectively duplicate packets or only do so when the Internet path performance is below a certain requirement. 
Similarly, other deployment scenarios (\S\ref{subsec:deployment}) may become more relevant if the cellular provider employs a usage-based pricing model. 

%ucharges based on the usage rather than the 
%depending on the deployment scenario (\S\ref{subsec:deployment}) as well as the pricing model of the cellular provider  a provider may not charge for extra bandwidth usage. 
%

%



\paragraph{Duplicating traffic has negligible impact on power consumption.} We tested the effect of duplicating a traffic stream on the battery life of the device. We ran 20 minute trials of Skype video calls, with and without cloud path duplication. We observed that in both cases the battery drain was $\sim$20 mAh, highlighting that the extra overhead of \sys{} has negligible impact on battery life. 

%We also observed that when the device is left idle for 20 minutes, the battery drain was $\sim$5 mAh. This indicates that while %increased network activity contributes to power consumption, duplicating a stream does not significantly increase the battery drain.

%Due to per-user, round-robin scheduling at cellular base stations and typically a large amount of packet buffering
\paragraph{Recovery is feasible despite latency issues.} Mobile networks also suffer from greater end-to-end latency and jitter~\cite{sprout2013}. We conducted a short study to quantify this effect by pinging three major cloud providers (Amazon, Microsoft, and Google) 1,000 times using different mobile networks: Verizon's LTE network (east coast) and T-Mobile's LTE network (both east and west coasts). %Pings from these networks took slightly longer than the home user latencies observed in \S\ref{sec:motivation} and had greater jitter. 
The median ping times to each provider was typically in the range of 50-60 ms, but the 50\%-90\% RTTs to each cloud provider was in the range of approximately 50-100 ms.

These latencies could be problematic for mobile receivers, as the effect of greater latency is multiplied in cooperative recovery. However, we observed that a Skype stream can be recovered during an outage,
using four mobile receivers, we see similar PSNR scores as fixed line (Figure~\ref{fig:rewan_skype_eval}). This is because Skype is able to adapt to greater end-to-end delay when recovery occurs over a longer duration.%long period of time.  
 Due to increased jitter, correcting random packet losses may be difficult for interactive applications, but can likely be mitigated for other applications (such as web transfers) using in-stream coding.

%Mobile networks have seen significant performance improvements in the past %decade~\cite{huanglte2013}: the transition from 3G to LTE cut latency and jitter by roughly half and %increased available bandwidth by $\sim$10x. New standards already deployed (LTE Advanced) and in the %pipeline (5G) will further improve mobile network performance. In the meantime, using \sys{} with %mobile networks is feasible, but may require selective transmission of data at the sender and/or %heavier coding on the inter-DC path to make up for bandwidth and latency issues, reducing %cost-effectiveness.

\subsubsection{Duplication Strategies}
%\paragraph{Sender Overhead.}
\label{subsec:deployment}

Our focus in this paper has been on scenarios where it is feasible for the sender 
to duplicate packets; we now explore strategies where this may not be feasible. 
%The following deployment scenarios determine \emph{who} duplicates the packets (and sends them to the packet recovery service) and \emph{which} packets are duplicated. Two possible scenarios could be:

\noindent\textbf{Selective Duplication.} When full duplication at source is infeasible -- due to limited access bandwidth or applications with high bitrates -- we can use \sys{} only for selected packets. To demonstrate the feasibility of such a strategy (and its potential benefits), we modify our TCP experiment (\S\ref{subsec:rewan-tcp-eval}) and only duplicate SYN-ACK packets. We observe that selective duplication reduces tail by 33\% (83\% with full duplication). Other examples of such duplication can include I-frames for video streaming, important user actions for gaming or AR applications, and the last packet of a window for short TCP transfers~\cite{gentleaggression}

\noindent\textbf{Duplication inside the network.} Another strategy, which requires support from the network, involves setting a bit in the packet header (e.g., TOS), which could indicates whether packet recovery is required or not. Based on this bit,
%the value of this bit, 
the ISP could duplicate the packet and send it to the cloud for packet recovery. Similarly, this duplication can also happen at a nearby data center, which can send the original packet through the public Internet and use the cloud path for coded packets only.
Finally, the network can also duplicate and send the copy to an alternate replica, if the other end-point application is replicated
across multiple sites/servers~\cite{rans-hotnets, tail_at_scale}. 


\begin{comment}
\begin{enumerate}[leftmargin=*]
    \item \emph{Selective Duplication at Source.} When full duplication at source is infeasible -- due to limited access bandwidth or applications with high bitrates -- we can use the packet recovery service 
    only for selected packets.  Examples include I-frames for video streaming, important user actions for gaming or AR applications, and the last packet of a window for short TCP transfers~\cite{gentleaggression}. We
    \item \emph{Duplication inside the network.} Another strategy, which requires support from the network, involves setting a bit in the packet, (John:  confusing, not specific enough.  which packet header?) which indicates whether packet recovery is required or not. Based on the value of this bit, the ISP could duplicate the packet and send it to the cloud for packet recovery. Similarly, this duplication can also happen at a nearby data center, which can send the original packet through the public Internet and use the cloud path for coded packets only.
\end{enumerate}
\end{comment}



\begin{comment}

\begin{table}[]
\centering
\scriptsize
\begin{tabular}{@{}ccc@{}}
\toprule
Coding Rate & Internet +  Overlay & Internet \\ \midrule
2/10 &  &  \\ \midrule
4/10 & 98\% & 100\% \\ \midrule
6/10 & 98\% & 100\% \\ \bottomrule
\end{tabular}
\caption{Median Packet Recovery Rates for cross-stream coding. Recovery gains diminish as coding rate increases. Internet $+$ Overlay has losses on both direct and overlay paths. Internet only has losses on direct path}
\label{tab:coding-overhead}
\end{table}

%\subsection{Inter-Data Center Bandwidth Overhead}
%\label{subsec:parameter-eval}
%In our previous experiments, we use a cross-stream coding rate of $r = 2/k$ where $4<=k<=6$ and in-stream rate of $s = 1/5$. While this rate might be acceptable for some applications, our goal here is to show that we can reduce this overhead and still provide adequate %recovery. In this experiment, we limit our overall coding overhead to 20\% by only using cross-stream coding with higher value of $k$ (10 in this case) and ignoring in-stream coding. We use 10 sources in Emulab and use similar topology as our TCP experiments. We send UDP %packets after every 10ms and perform two iterations. In our first iteration, we only introduce losses on direct Internet path, whereas in our second iteration, we have losses on overlay path as well. 
%Table~\ref{tab:coding-overhead} shows that by using low $r$ i.e. 20\% overhead, we are able to recover X\% of lost packets on all paths. We are able to achieve even higher recovery rates by increasing overhead to 40\% ($r=4/10$), however, we also increase inter data center %bandwidth overhead. %This shows that applications can rely on cross-stream coding only to further reduce cloud bandwidth costs.















\begin{figure}[!t]
 \centering
 \includegraphics[width=3.2in]{graphs/coding_rate.pdf}
 \caption{Recovery gains diminish as coding rate increases. Internet $+$ Overlay has losses on both direct and overlay paths. Internet only has losses on direct path.}
 \label{fig:coding_rate}
\end{figure}

\end{comment}

\begin{comment}
\subsection{Coding Rate Selection}
\label{subsec:parameter-eval}
In \sys{}'s design, coding rate ($r = 2/k$), plays an important part in determining packet recovery performance as well as inter data center bandwidth overhead. In this experiment, we show that by varying coding rate, we can adjust bandwidth overhead and recovery accuracy according to application demand.

We use similar topology as our TCP experiments but send UDP packets from 20 sources after every 10ms. We use $k=20$ and vary $r$ by increasing cross-stream coded packets.
We ignore in-stream coding in this case as it has limited benfits for high $k$. For coding rate, we start with $r = 2/20$ and subsequently increase to $4/20$, and $6/20$.  These values correspond to $10\%$,$20\%$ and $30\%$ inter data center packet overhead.

We perform two iterations of 1 hour each for these rates and send approx 360k packets from each source. In our first iteration, we only introduce losses on direct Internet path, whereas in our second iteration, we have losses on overlay path as well. Figure~\ref{fig:coding_rate} shows that by using low $r$ i.e. 10\% overhead, we are able to recover 84\% of lost packets on all paths. We are able to achieve high recovery rates by increasing overhead to 20\% ($r=4/20$), however, we do not get much improvement if we increase it any further. One thing to note is that by lowering cloud bandwidth overhead, we are increasing receiver side bandwidth usage (X\% in this case), as it has to respond to large cooperative requests. Since cooperative requests are very small in size, bandwidth cost at DC2 are not increased by much.
\end{comment}


























\begin{comment}

\osama{placement is not final, neither is text}
We now perform back of the envelope calculations to estimate cost of deploying 
\sys{} and compare it to a solution that fully uses cloud overlay. Based on above results, we calculate bandwidth usage of a single HD Skype call to be 0.675 GB per hour. So, for a single \sys{} thread, that handles 150 HD calls in an hour, DC1 will receive 101.25 GB data. Assuming DC1 is in US, where Azure charges \$0.087 per GB for egress traffic, cost of forwarding all traffic using a single overlay node comes out out to be \$8.8 per hour. Using a coding rate of $1/5$, this cost is reduced to \$1.76 per hour. Therefore, cost of bandwidth is much lower when using \sys{}. Meanwhile, Azure's compute cost for a single core, D-type, general purpose machine is \$0.073 per hour. Hence, compute charges are low as compared to bandwidth cost.
\end{comment}
%If \sys{} coding rate is $r = 1/5$, DC1 will send 20.25 GB of data on egress towards DC2. Assuming DC1 is in US, for Azure, egress cost is $\$0.087$ per GB, total bandwidth cost comes out as \$1.76
%shows that ReWAN could be used within the context of NFV. \cody{How? And is this the place for this exposition, or should that be saved for %Discussion?}


\begin{comment}
\subsection{\sys{} Real Network Performance}

\paragraph{Objective:} 
Run \sys{} on real network to see its actual performance

\paragraph{Approach:}

\begin{itemize}
    \item Replay Skype traces/CBR on PlanetLab
    \item Compare against cloud based overlay
    \item Plot network level metrics (packet recovery time & recovery overhead)
\end{itemize}






\osama{First, I will identify other solutions that we want to compare against. Then I will outline the metrics that we will be looking at, they will further be divided into cost-benefit categories}\\


\textbf{Comparison}
\begin{itemize}
    \item Cloud based full overlay
    \item Public Internet with end to end fec
\end{itemize}

Our scheme should have benefits of cloud based overlay and cost of best-effort public Internet. For cloud based overlay, the benefits are high but costs are high as well. If using public Internet with additional FEC, the benefits are low as well as cost is low.\\

\textbf{Metrics}
\begin{itemize}
    \item User level: PSNR, MOS, bandwidth cost
    \item Network Level: Packet recovery time, packet (bandwidth) overhead
\end{itemize}

In terms of benefits and costs, 
\begin{itemize}
    \item Benefits : high PSNR \& MOS for tail, recovery times < 150ms
    \item Cost : bandwidth costs and additional packet(bandwidth) overhead
\end{itemize}
\osama{Im still working on precisely defining cost and packet overhead}



\textbf{Network Environment}
We will have three network environments,
\begin{itemize}
    \item Testbed with Skype integration
    \item Emulated (Emulab) setup for large scale analysis
    \item Real Network: PlanetLab
\end{itemize}
For Testbed and Emulab, we will have realistic loss \& delay patterns based on measurements. These patterns could also be modeled.\\

\textbf{Applications}

For applications, we will have
\begin{itemize}
    \item Skype running over testbed
    \item Skype trace replay over Emulab \& PlanetLab
\end{itemize}
I'm not sure if constant bitrate application will benefit us, as the paper is more focused towards interactive low data rate applications.

\subsection{EXP 1: Skype with \sys{}}

This experiment will show how \sys{} works under realistic settings, it will be a follow up to section 2 Skype testbed experiment. We will look into user level metrics with focus on bad frames and compare with other schemes as well. We can also divide \sys{} into three subparts with FEC only, NC only, FEC + NC.

\subsection{EXP 2: Large scale behavior}

The purpose of this experiment is to show how much benefit, we will get when we run \sys{} on large scale. 

We will have a topology with 50-100 nodes on emulab, and will replay skype traces. We will model loss and delay patterns from our measurements and compare network level metrics against other techniques along with cost comparison.


\subsection{EXP 3: \sys{} parameter tuning}
This experiment will show, how much \sys{} performance is sensitive to different parameters. We will run it on EXP 2 topology and see how much \sys{} performance varies. We identify following key parameters.
\begin{itemize}
    \item DC1 timer and/or coding block size
    \item Additional Network Coded packets for stragglers
\end{itemize}


\subsection{EXP 4: \sys{} on Real Network}

This experiment will show how \sys{} fares in real network. We replay skype traces on Planetlab with \sys{} and try to see how much actual gains are there.


\end{comment}


==> ReWAN-arxiv(1)/implementation.tex <==
\section{Implementation}
\label{sec:implementation}
We now describe how to coordinate clients and data centers in practice, and elaborate on the prototype that we built to evaluate \sys{}.

\subsection{Bootstrapping \sys{}}

\paragraph{Data Center Selection.}
Before any communication can take place in \sys{}, senders and receivers must learn about their nearest \sys{}-enabled data center. On boot, a client only has knowledge of a master data center or web service, which it contacts to determine the location of this nearest data center. Optimally, the ``nearest'' data center will be the one with the lowest latency to the inquiring client, since our goal is to provide timely packet recovery. %Initially, IP geolocation services can help provide an acceptable approximation of a close data center. %\textcolor{red}{, but \sys{} could also maintain its own statistics about latencies to data centers from previous streams to serve more suitable data centers to new clients.}

\paragraph{Clients Joining \sys{}.}
Once a client is ready to send data using the \sys{} service, it uses a control channel to contact its nearest data center (DC1) to set up a cloud overlay path. DC1 must then select an acceptable receiver-side data center (DC2), which it can do using the same data center selection methods. The chosen DC2 node must be close to the receiver in order for recovery to work within a time budget.
%\textcolor{red}{When joining \sys{}, at a minimum, clients must specify the endpoints of the communication and the duration of service to be able to choose a relevant DC2 node and maintain data structures for the flow. Clients may also specify additional information that enables \sys{} to make more informed coding, loss detection, and loss recovery decisions, such as the maximum acceptable loss rate or latency as well as the expected data rate of the stream.} % For example, DC2 may choose to abstain from cooperative recovery if it deems the recovery to be too late or if a loss would be acceptable in terms of the overall loss rate.
%
%\john{Do we have any DDoS defense?  %Looks very easy to take out ReWAN as %specified.}
%I assume not.
 DC1 and DC2 will provision the necessary resources and alert the sender that it may begin sending. From that point, the sender can begin transmitting data to DC1 for \sys{} 
to use as input for encoding over the cloud overlay path. 

\subsection{\sys{} Prototype}

The \sys{} prototype is implemented in C++ and operates in user space. 
Our implementation uses UDP for forwarding application traffic, coded packets, and cooperative recovery packets, and uses TCP for control channel traffic between the endpoints and the data centers. Applications can utilize \sys{} in two ways. First, iptables~\cite{iptables} and the NetFilter library~\cite{netfilter} can be used to install forwarding rules designed to ``catch'' outbound application traffic, redirect it to \sys{} to duplicate it on the data center path -- we use this for closed-source applications like Skype, where we are not at liberty to modify packets before they are transmitted by the application. Alternatively, \sys{} can act as a proxy listening on a local port for applications to directly send data. The data is received and encapsulated in the \sys{} header before being sent to the destination and DC1.
\begin{comment}
 

 \begin{figure}[!t]
\centering
 \includegraphics[scale=0.20]{figures/packet_header.png}
 \caption{\sys{} base packet header}
  \label{fig:pkt-hdr}
\osama{change the figure to save space}
 \end{figure}

\end{comment}

%\sys{} implementation is split into several modules, which can be divided into
%two main categories, node specific and general. A node specific module only uses components relevant to the role
%of the node in the overall topology. A sender node only uses sender module whereas receiver node only uses receiver module, similarly DC1 and DC2 use their respective modules to handle incoming data.
%General modules are used by each node and are common across board, these include coding, logging, debugging, generic sending and receiving libraries.

%\begin{comment}


A \sys{} packet is essentially a UDP packet with application data packet as payload. \sys{} has a basic 32 byte header containing
standard flow fields.
%%that contains the following fields,
%% JB:  ugly, needed?
%%\texttt{\{type (2), len (2), seqno (4), src (9), dst (9)\}}. 
Based on the type of packet, the header may include extra information. For example, an application data packet will include only the base header, whereas a coded packet will include information about how many flows are encoded, which flows are encoded, and which sequence numbers are involved. Similarly, cooperative recovery request and response packets contain information about the requested and lost packets.
%\end{comment}

Our prototype uses Reed-Solomon codes to encode and decode application data using the open-source zfec~\cite{zfec} library, and uses %$\alpha$=0.5 for weighted timer, 
25ms for the small timer and RTT for the long timer.
%uses a standard dynamic timeout mechanism $T$ for loss detection, calculated as: $ T = \alpha \times \lambda_{new} + (1-\alpha) \times T $. New inter-arrival times are factored in with a weight $\alpha$, which we set to 0.5. 
Proactive loss detection mode is triggered with a string of three consecutive NACKs, similar to the TCP best-practice of triple duplicate ACKs. Finally, we tune the parameters related to coding (coding rate, timers, and queues) on a per-application basis, depending on the application's characteristics and requirements.

==> ReWAN-arxiv(1)/intro.tex <==
\section{Introduction}
\label{sec:intro}

Notable in an era of constant change, the Internet of today retains a 40-year old design philosophy built around the principle of a ``stupid network'' with smart endpoints.  Today's IP network layer offers best effort service, with no guarantees on latency, packet loss, or bandwidth; while important functions like reliability and congestion control continue to be implemented at the end-points, as part of the TCP transport.  This is despite well known pain points in many scenarios -- for example, recent studies again highlight how network problems lead to problems for latency sensitive applications, such as streaming~\cite{qoe1, qoe2} and short web-transfers~\cite{gentleaggression}.
With the emergence of virtual reality (VR) and augmented reality (AR) applications, the demands on the network continue to increase and apply pressure to the underlying architecture.

%applications often require \emph{richer} network services (e.g., multicast~\cite{esm}, resilient %routing~\cite{ron, detour}) to meet their objectives. 

%Unfortunately, introducing any change inside the network is difficult. New functionality is often %implemented in an ad hoc fashion -- such as application-specific middleboxes or overlays -- which %makes the Internet fragile, and limits performance and innovation. As a result, applications often %fall short of meeting their quality of service (QoS) objectives -- recent studies highlight how %network problems lead to user dissatisfaction for video streaming applications~\cite{qoe1, qoe2}.
%With the emergence of virtual reality (VR) applications, the demands on the network will only increase %in future. 

% \vspace{0.1in} 
%\noindent \textbf{Emergence of Virtual Reality Applications and the Cloud.}
%The long standing dream of virtual reality (VR) applications is finally becoming a reality. VR devices (e.g., Oculus Rift) %are already in market, and there is tremendous interest in developing VR applications that can transform user experiences, in %areas as diverse as education and shopping, to communication and gaming. 
%These applications will put even more demands on the network: they typically require high bandwidth (typically due to use of %multiple high-definition cameras), extremely low latency (to maintain interactivity), and significant amount of computation %(e.g., computer vision algorithms). We need networks that can support these requirements! 

Fortunately, the emergence of \emph{the cloud} offers us a new opportunity to better support the needs of latency sensitive applications without re-architecting the underlying best effort Internet. By the cloud, we refer to a distributed network of data centers (DCs), inter-connected through a private network (e.g., Azure, EC2, Google Cloud).  For any communication between two end-points, we can potentially use the cloud as an \emph{overlay}, with DCs acting as an insertion point for in-network services~\cite{rewanhotnets, via2016}. A cloud-based overlay offers unique opportunities: cloud paths are well-provisioned, offering low jitter and very high reliability; and each DC has visibility into many users and applications, so it can act as a unique vantage point for control. On the flip side, using the cloud as an overlay can be costly: cloud providers charge for the use of their resources (e.g., processing, network connectivity), with wide area network (WAN) bandwidth being particularly expensive~\cite{swan, eurosys15, rewanhotnets}. Therefore, we argue that the most effective use of the cloud as an overlay is one that does so in a \emph{judicious} manner. 

In this paper, we design, implement, and evaluate \sys{}\footnote{Cloud ASsisted Packet Recovery (\sys{}).}, a packet recovery service for latency-sensitive applications operating on the wide-area best-effort Internet. \sys{} uses the cloud overlay \emph{only} for packet recovery: it sends a low rate of \emph{coded} packets across the inter-DC paths; these coded packets are used only in case of a packet loss on data transmitted along the best effort Internet path. 
The coded packets provide resilience to a wide range of common packet loss and jitter scenarios, e.g., both random and bursty losses, and packets experiencing high delay. At the same time, it makes economical use of the expensive inter-DC bandwidth. The two key pieces of \sys{}'s design are the \emph{coding scheme}  and the receiver-driven \emph{cooperative recovery protocol}, described next.


\begin{comment}
In this paper, we design, implement, and evaluate \sys{}\footnote{Cloud ASsisted Packet Recovery (\sys{}).}, a packet recovery service for today's best-effort  Internet. \sys{} uses the cloud overlay \emph{only} for packet recovery: it sends a low rate of \emph{coded} packets across the inter-DC paths; these coded packets are used only in case of a packet loss on data transmitted along the best effort Internet path. 
The coded packets provide resilience to a wide range of common packet loss and jitter scenarios, e.g., both random and bursty losses, and packets experiencing high delay. At the same time, it makes economical use of the expensive inter-DC bandwidth. The two key pieces of \sys{}'s design are the \emph{coding scheme}  and the receiver-driven \emph{cooperative recovery protocol}, described next. 
\end{comment}
% s is already used for in-stream coded packet rate.
Using \sys{}, each packet sent on the public Internet path is additionally routed to the source's nearest ingress DC.  Each ingress DC
then determines a coding plan on-the-fly based on the arrival of all packets to that DC.  
Packets destined to the same destination region -- with a common {\em egress DC} --  that arrive within a short window of time
are grouped together to form
%% too much emph
%%a \emph{batch}, 
a batch, over which coding occurs. For each batch of $b$ packets, \sys{} generates a set of encoding packets at a tunably low rate $r < 1$, so that $rb < b$ packets are computed and transmitted along the DC-DC path and protect each batch of $b$ best-effort transmissions.  Encoding is done in two complementary forms:  cross-stream coding encodes packets \emph{across} user streams, while in-stream coding encodes packets \emph{within} a single flow.  The latter provides protection against random losses, while the former can protect against burst losses or even a sustained outage along a best-effort path, as we demonstrate shortly.



%Packets are grouped by their {\em egress DC}, i.e., all packets headed to destinations in the same region are partitioned into a group for that egress DC.
%Within this group, all packets arriving during a short window of time 
%form a \emph{batch}, over which coding occurs.  For each batch of $b$ packets, \sys{} generates a set of encoding packets at a tunably low %rate $r < 1$, so that $rb < b$ packets are computed and transmitted along the DC-DC path and protect each batch of $b$ best-effort %transmissions.  Encoding is done in two complementary forms:  cross-stream coding encodes packets \emph{across} user streams, while in-stream %coding encodes packets \emph{within} a single flow.  The latter provides protection against random losses, while the former can protect %against burst losses or even a sustained outage along a best-effort path, as we demonstrate shortly.


\sys{} uses a receiver-driven mechanism to initiate and cooperatively recover from packet loss. 
%First, the onus of detecting a loss is on the receiver, where existing techniques based on missing sequence numbers and timeouts to detect a %loss (or delayed packet) are used. 
%\john{I think these next few sentences are too much detail for the intro, not especially novel.}
%The rationale behind this is that the receiver is in the best position to know its requirements as well as its capabilities. A receiver may elect not %to initiate recovery for all lost packets; alternatively, it may request recovery using a different, but typically expensive interface, such as %cellular. 
%\john{end proposed cut}
To initiate recovery, the receiver notifies the egress DC about the missing packets.  The egress DC consults the coding plan to determine the right recourse for recovery -- forwarding in-stream coding packets while sufficient and failing over to 
%% too much emph
%\emph{cooperative recovery}
cooperative recovery
 when necessary. For packets requiring cooperative recovery,  the egress DC must gather the rest of the batch: the cross-stream packet(s) plus the data packets from other receivers.  
 %While this entails extra overhead, the use case is not primarily to recover from single losses (handled by in-stream coding), but to recover from a burst loss, or indeed, a sustained outage. 
 %In this case, a pipelined decoding process, potentially spanning multiple batches, is established at the DC.  
 Our cooperative recovery mechanism exploits today's cloud bandwidth pricing model, in which incoming bandwidth is typically free~\cite{amazonprice,azureprice,googleprice} -- so recovery incurs relatively low bandwidth cost as receivers send their data packets to the DC using the free ingress bandwidth. 
%\osama{changes required here}

We have implemented \sys{} as a network layer service that intercepts transport segments and performs recovery as described above, 
seamlessly working with both TCP and UDP based applications without requiring any application modification. 
We have deployed \sys{} as a service on a public cloud for over a month and measured the wide area performance of PlanetLab paths. Our results show that \sys{} is able to recover more than 70\% of losses, the recovery is typically within half a round-trip time (RTT),
and the overhead of using the cloud judiciously is far less than a traditional overlay solution that uses the cloud exclusively.
Through controlled experiments, we also evaluate how \sys{} interacts with protocols up and down the network stack -- we show that: i) \sys{}'s packet recovery can improve the user's QoE experience for a skype video conferencing scenario, ii) \sys{} can speed up short web transfers by avoiding TCP timeouts and congestion avoidance caused by bursty losses, iii) it is feasible to use \sys{} on mobile networks, in terms of bandwidth, energy consumption, and latencies to nearby DCs.

%\john{What I like about these thrusts are the ``up and down the network stack'' angle I tried to convey in the abstract.}

%LTE networks offer sufficient bandwidth and and future's cellular  showing  its negligible impact on battery consumption, 
%and the increasing available bandwidth and decreasing latency between end-users and their nearby data centers because of LTE
%to make \sys{}'s packet recovery effective. 


%We also show that running \sys{} on top of TCP reduces tail latency of short flows by x\%. 
%Moreover, we also show that \sys{}'s benefits translates into improvement in user-perceived metrics for Skype's video conferencing scenario %under realistic network conditions \osama{say something about mobile and fixed here}.  

%Our evaluation is done on a small testbed, using a combination of real and synthetic application traces. We emulate real network %conditions using path loss and delay traces obtained from wide area PlanetLab paths. 
%Our evaluation shows that \sys{} provides fast recovery, which is comparable to sending all packets using the cloud overlay, while %requiring
%only a fraction of bandwidth compared to the traditional overlay based approach. 
%\fahad{eval para needs to be updated}

Overall, we make the following contributions in this paper. 

\begin{itemize}[leftmargin=*]
    \item A case for judicious packet recovery by sending only coded packets across the inter-DC path. 
    
    \item A design and implementation of \sys{}, including a practical, tunable coding module and a receiver-driven protocol for cooperative packet recovery. 
    
    \item A multi-faceted evaluation of \sys{}, using both network and user level metrics, on diverse networks (PlanetLab, cellular) and applications (video conferencing, short web transfers).
    
    %and two popular cateogry of applications on a public cloud with wide area PlanetLab paths, an evaluation of \sys{} for Skype's video %conferencing scenario\textcolor{blue}{, and an evaluation of \sys{}'s effectiveness in a mobile setting}. \osama{revise this to include %tcp, something in terms of protocols and networks}
    
    
\end{itemize}


%\sys{} can deal with a range of packet loss scenarios (e.g., random, bursty, etc) while making judicious use of the cloud %resources (i.e., inter-DC bandwidth). At the heart of \sys{} is a practical \emph{coding} scheme which uses  

==> ReWAN-arxiv(1)/motivation.tex <==



\section{Motivation}
\label{sec:motivation}
%In this section, we make a case for judiciously using cloud as an overlay for applications running over public Internet paths. We first show %how latency sensitive applications suffer from poor network performance.% despite built-in reliability mechanisms.
%We then describe how a cloud based overlay can overcome shortcomings of today's Internet.
%\fahad{I would suggest focusing on the network scenario more than the applications. You can just list the applications, but talk more about the well connected end-points (which can afford to send redundant data) and the problem of losses in the middle}

%\osama{narrowing the focus, this small section should address main criticism from previous reviews %i.e. where can it be used? sender access overhead}

\subsection{Problem Description}
\label{subsec:prob-desc}
Our focus is on latency-sensitive applications, such as video chat, collaborative AR/VR, and short web transfers. Unfortunately, network impairments, such as packet loss and jitter,
 still remain a problem for these applications. Recent studies show how poor network conditions impact the user experience for popular applications. 
For example, Microsoft's analysis of 430 million Skype calls reveals that network conditions such as round trip time (RTT), loss rate, and jitter are directly correlated with perceived user experience~\cite{via2016}. They observe that poor network conditions impact 15\% of calls, with wide area paths being 2-3x more prone to poor network conditions. Similar problems have also been observed for short web transfers~\cite{gentleaggression}. 

%by Google shows that 10\% of TCP connections lose at least one packet and losses can increase average %flow completion times by up to 5x for web transfers. 
 
While network problems can be of different types, we focus on 
the particularly challenging scenario of impairments in the ``middle'' for wide-area paths -- paths with high round-trip time between them (e.g., across continent, east-west coast, etc).
For such wide-area paths, even if the two end-points have good access network connectivity (e.g., enterprises, universities, etc) -- as we assume in this paper --  they still have to rely on the best effort Internet (or the ``middle''), which can experience poor performance due to various issues in the core (e.g. routing misconfigurations~\cite{arrow}, peering disputes~\cite{congestion-imc14}, router/link failure~\cite{ron,arrow}, etc). 


\paragraph{Limitations of Existing Solutions.}Several prior proposals, from the seminal work on RON~\cite{ron}, to recent proposals like Arrow~\cite{arrow}, also focus on this problem of network impairments in the ``middle''.
However, solving this problem is challenging. 
Simple retransmission based techniques (e.g., TCP), as well as edge proxy solutions~\cite{tapaconext, Bakre97, catnap, DogarM208}, have limited benefits given our target application and network settings (latency sensitive applications, wide area paths, losses in the middle, etc). 

Redundancy-based solutions (e.g., FEC) 
are more applicable, but unfortunately cannot cope with burst losses or outages that can occur on wide area Internet paths. Previous measurement studies as well as our experiments show that such bursty losses and outages can last for seconds~\cite{ron, rewanhotnets}. Other proposals (e.g. Maelstrom~\cite{maelstrom}, Raptor~\cite{raptor}) use layered interleaved coding to provide protection against bursty losses, but their reliance on future packets adds non-tolerable delay for latency sensitive applications. 

Finally, overlay networks, such as RON~\cite{ron}, can potentially avoid these bursty losses and outages on the direct Internet path by taking alternate (overlay) paths. However, traditional overlay networks have to deal with problems of node churn and lack of performance predictability, which limit their practical use for performance critical applications. 


\begin{comment}
Interactive applications can potentially use aggressive redundancy techniques to cope with packet losses. For example, Skype uses \emph{aggressive FEC} to mask packet losses; similarly other proposals \emph{duplicate} packets during slow start of TCP to reduce the flow completion times of TCP flows~\cite{gentleaggression}. Unfortunately, such techniques cannot cope with burst losses or outages that can occur on wide area Internet paths. Previous measurement studies as well as our experiments show that such bursty losses and outages can last for seconds~\cite{ron, rewan-anon}. Other proposals (e.g. Maelstrom~\cite{maelstrom}, Raptor~\cite{raptor}) use layered interleaved coding to provide protection against bursty losses; however, these schemes do not provide fast enough recovery for interactive applications. Their reliance on future packets adds non-tolerable delay for latency sensitive applications.






%\end{Comment}
\textcolor{red}{
\paragraph{Application and Network Scenarios.}
Our focus is on latency-sensitive applications (e.g. video chat, collaborative AR/VR) that operate in an \emph{enterprise} network setting. While larger enterprise organizations (e.g., universities, mid-size corporations) are very well-connected, they still rely on the best-effort Internet to fulfill quality of service requirements. Latency-sensitive applications on these networks suffer from poor performance due to various issues (e.g. routing misconfigurations~\cite{arrow}, peering disputes~\cite{congestion-imc14}, router/link failure~\cite{ron,arrow}) in the core. Our work addresses these problems by utilizing public cloud infrastructure, complementing previous proposals (Arrow~\cite{arrow}, RON~\cite{ron}). 
%modern and future (e.g. collaborative AR/VR) applications.
We believe it is a natural fit for enterprise networks that have well connected end-points and can afford to send some redundant data without incurring significant extra bandwidth costs.
}





\paragraph{Problems with Latency Sensitive Applications.} Despite decades of research, network impairments, such as packet loss and jitter,
%% too much emph
%%\emph{still} 
still remain a problem for latency sensitive applications. 
Recent studies show how poor network conditions impact the user experience for popular applications. 
For example, Microsoft's analysis of 430 million Skype calls reveals that network conditions such as round trip time (RTT), loss rate, and jitter are directly correlated with perceived user experience~\cite{via2016}. They observe that poor network conditions impact 15\% of calls, with wide area paths being 2-3x more prone to poor network conditions. Similar problems have also been observed for web transfers. A 2014 study~\cite{gentleaggression} by Google shows that 10\% of TCP connections lose at least one packet and losses can increase average flow completion times by up to 5x for web transfers.  
%\fahad{can we have better/more concrete supporting evidence from these papers?}
%longer to complete as compared to optimal time. The reason for this delay is that 77\% of losses are recovered by TCP via RTO. Additionally, %due to short nature of these flows, most of the losses occur at the end of window. 




%but that a managed overlay architecture consisting of globally distributed relays can significantly improve network performance and, %consequently, user QoE. For example, carefully assigning a subset of calls to use the relay path can improve Skype audio call quality by 
%45\%. 

%\paragraph{Long tail of request-response web services}

%Another source of long tail is the delay added by the mobile networks. A flow running through a typical 3G network would experience delays %in hundreds of milliseconds~\cite{hpbn}. While these delays have been reduced due to recent LTE deployments, they still are a significant %factor in tail.



%\subsection{Cloud as an Overlay}
%\label{subsec:cloud_motiv}

\paragraph{Limitations of Existing Solutions.} %\fahad{Mention here why even aggressive FEC %doesn't work; perhaps also mention %overlay-based solutions like RON}


Interactive applications can potentially use aggressive redundancy techniques to cope with packet losses. For example, Skype uses \emph{aggressive FEC} to mask packet losses; similarly other proposals \emph{duplicate} packets during slow start of TCP to reduce the flow completion times of TCP flows~\cite{gentleaggression}. Unfortunately, such techniques cannot cope with burst losses or outages that can occur on wide area Internet paths. Previous measurement studies as well as our experiments show that such bursty losses and outages can last for seconds~\cite{ron, rewan-anon}. Other proposals (e.g. Maelstrom~\cite{maelstrom}, Raptor~\cite{raptor}) use layered interleaved coding to provide protection against bursty losses; however, these schemes do not provide fast enough recovery for interactive applications. Their reliance on future packets adds non-tolerable delay for latency sensitive applications.

Overlay networks, such as RON~\cite{ron}, can potentially avoid these bursty losses and outages on the direct Internet path by taking alternate (overlay) paths. However, traditional overlay networks have to deal with problems of node churn and lack of performance predictability, which limit their practical use for performance critical applications. 
\end{comment}
%as the peer nodes and their paths typically offer best-effort service. 
%previous studies show that such best-effort overlays typically recover only 40-50\% of lost packets~\cite{detour,cloudstudy-www}.


\begin{comment}

\begin{figure*}[!t]
%\centering
  %\hspace{-2em}
  \hspace*{\fill}
  \subfigure[\small reactive]{\includegraphics[width=1.6in]{figures/reactive.png}\label{fig:reactive}}\hfill
%\hspace{2em}
  \subfigure[\small corrective]{\includegraphics[width=1.6in]{figures/corrective.png}\label{fig:corrective}}\hfill
 %\hspace{2em}
  \subfigure[\small proactive]{\includegraphics[width=1.6in]{figures/proactive.png}\label{fig:proactive}}
 \hspace*{\fill}
  \caption{Cloud Overlay for Packet Recovery}
 \end{figure*}

\end{comment}
\subsection{The Cloud as an Overlay}
\label{subsec:cloud-overlay}
We consider using a cloud overlay as a potential solution to our problem. Some interactive applications, such as Skype and Google Hangout, are already migrating their services to at least partial use of cloud relays~\cite{via2016}, but there has been little work in studying how to best utilize the cloud for these types of interactive communications. Therefore, we characterize the properties of cloud paths in terms of network conditions and cost, and ask:
%the following question
can the cloud be leveraged in a cost-efficient way to make up for the Internet's performance limitations?


\emph{Benefits.} There are several advantages of using the cloud as an overlay. First, measurements show that cloud paths are highly reliable with a typical downtime target of a few minutes per month~\cite{goog-avail, cloudstudy-www}. A recent study shows that inter data center paths have an order of magnitude lower loss rate, and significantly higher bandwidth, compared to public Internet paths~\cite{cloudstudy-www}. Similar benefits are being extended all the way up to ISP networks, with major cloud operators providing bandwidth-guaranteed pipes between their data centers and customer premises (e.g., Azure ExpressRoute~\cite{azure-expressroute}, AWS Direct Connect~\cite{aws-direct-connect}).  These advances are poised to make the \emph{entire} cloud overlay highly reliable, including both the WAN as well as the last hop to the end-users.  
%A recent measurement study shows that wide area cloud paths have availability of three 9's whereas average Internet paths have %availability of only two 9's~\cite{interdcpathstech2016}. 
Second, cloud infrastructure provides the ability to implement in-network services in software in a  scalable and fault tolerant fashion, with the help of network function virtualization (NFV)~\cite{combsekar2012,middleboxsherry}. 
Third, cloud operators also strive to provide low latency access to end users, for example, by direct peering with customer ISPs to provide better and faster access to popular web services~\cite{goog-onehop}. 
Recent studies
%% JB:  not clear why relevant
%%, focusing on PlanetLab paths,
show that using cloud paths only adds a small amount of latency compared to that of the public Internet~\cite{middleboxcloud, rewanhotnets}.




\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[width=3.2in]{graphs/cloud_lat_new.pdf}
 \caption{Cloud latency from 500 random RIPE Atlas home nodes. 80\% of homes reach nearby cloud node within 35ms.}
 \label{fig:cloud-lat}
\end{figure}
\end{comment}


\begin{comment}


\begin{figure*}[!t]
\centering
  %\hspace{-2em}
  \subfigure[\small ISP]{\includegraphics[width=1.6in]{figures/isp.png}\label{fig:isp}}
\hspace{2em}
  \subfigure[\small selective]{\includegraphics[width=1.6in]{figures/selective.png}\label{fig:selective}}
 \hspace{2em}
  \subfigure[\small full]{\includegraphics[width=1.6in]{figures/full.png}\label{fig:full}}
  \caption{Duplication Strategies}
 \end{figure*}
\end{comment}

\begin{comment}
To validate this observation over a broader set of end-points, we quantify how fast home users all across the world can reach their nearby cloud. We conduct an experiment using the RIPE Atlas infrastructure~\cite{ripe-atlas} -- we randomly select 500 nodes (measurement devices), %located in homes/enterprises), 
spread all over the world, and ping popular websites hosted on the three major cloud providers. Figure~\ref{fig:cloud-lat} shows the CDF of the round-trip-time (RTT) observed by the nodes -- it shows that 80\% of the nodes can access a nearby cloud with an RTT of 35 ms or less, validating the hypothesis that using a cloud overlay is increasingly becoming a feasible option even for latency sensitive applications. 
\end{comment}
%We also conduct a small study where we ping these cloud providers using two different US mobile carriers. Figure~\ref{} shows that 50\% of time rtt is less than 70m.  These results as well as other studies~\cite{middleboxcloud, rewanhotnets} show that using cloud as an overlay will not add significant latency inflation on end to end path.

\emph{Cost.} Although the cloud as an overlay provides significant benefits, it can be expensive to use, especially due to the high cost of inter-DC bandwidth. 
%To demonstrate bandwidth cost, we do a back-of-the-envelope calculation for deploying a solution that uses cloud overlay. An interactive video calling application, based on the bandwidth requirement of 1.5Mbps~\cite{skype_bw}, sends 0.675GB of data per hour. A single data center node, in an overlay, will receive and forward approx 101GB of data per hour for 150 parallel application sessions. For a 2-node overlay node, based on today's cloud pricing~\cite{azureprice}, this would cost a minimum of \$17/hour for bandwidth and \$2/hour for general purpose compute usage. 
Anecdotal evidence, as well as our discussions with operators, suggests that an inter-continental leased line could be an order of magnitude or more expensive compared to a connection to the best effort Internet.
%% obvious, redundant.  just say best-effort (which offers no guarantees on the wide area paths). 
This reasoning underlies several recent proposals that try to make efficient use of inter-DC bandwidth in order to reduce their network costs~\cite{rewanhotnets,interdcpricing2016,netstitcher2011}. 
%Although the cloud as an overlay provides significant benefits, it can be expensive to use, especially due to the high cost of inter-DC bandwidth.%Anecdotal evidence, as well as our discussions with operators, suggests that an inter-continental leased line could be an order of magnitude or more expensive compared to a connection to the Internet (which offers no guarantees on the wide area paths). %This reasoning underlies several recent proposals that try to make efficient use of inter-DC bandwidth in order to reduce their network costs~\cite{rewan-anon,interdcpricing2016,netstitcher2011}. %Similarly, making efficient use of the wide aSeveral WAN optimization techniques like compression, de-duplication, and FEC are used to reduce %cost and increase utilization. Hence, a cloud based overlay service will incur significant bandwidth costs.
\begin{comment}
\begin{figure}[!t]
\centering
 \includegraphics[width=1.6in]{figures/solution-space.png}
 \caption{Reliability Solution Space Analysis}
 \label{fig:solution-space}
\end{figure}
\end{comment}

\paragraph{A Cloud-based Packet Recovery Service.}
We argue that in current settings, we only need to rely on the cloud whenever the best-effort Internet cannot provide the desired reliability. 
%\begin{wrapfigure}{L}{0.15\textwidth}
\begin{figure}[!t]
\centering
\includegraphics[width=1.4in]{figures/solution-space.png}
\caption{Reliability Solution Space Analysis}
\label{fig:solution-space}
%\end{wrapfigure}
\end{figure}
We propose \emph{judicious} use of cloud paths: leveraging the availability and performance of cloud only when the best-effort Internet encounters problems. 

Figure~\ref{fig:solution-space} shows why a judicious use of the cloud is desirable.
An Internet only solution has low cost but offers low reliability. 
In contrast, a cloud only solution offers high reliability, at the expense of higher cost. 
By judiciously using the cloud, we can approach the optimal line:  applications can rely on the public Internet to deliver most of the packets, and use the cloud to augment end-to-end availability. 
For example, an application using an Internet path with 1\% loss is still getting 99\% of its packets delivered, so it should sparingly use the cloud. 
Our proposed packet recovery service is an example of how this can be done: it uses the cloud \emph{only} for packet recovery. 

\begin{comment}
\textcolor{red}{
\osama{moved this section to here: inline with new story}
\paragraph{Deployment Model}
A packet recovery service can be used in variety of ways: it can potentially be deployed by the cloud infrastructure provider, an ISP, or a third-party service provider who pays the cloud operator only for the infrastructure usage. %Users can explicitly opt into using it if they require a more reliable packet recovery service -- for example, implemented as a paid service or added value proposition. The following deployment scenarios determine \emph{who} duplicates the packets (and sends them to the packet recovery service) and \emph{which} packets are duplicated. Three possible scenarios could be:
%This is the primary scenario that we focus on in this paper -- in this case, 
In our proposed scheme, the source duplicates every packet and sends a copy to the cloud for possible recovery at a later time. 
Given the relatively low bit rate of many latency-sensitive applications, and the high capacity of access links for enterprise networks, we claim that this strategy is feasible in many common scenarios. 
Our experiments also confirm the feasibility of this approach for a wide range of other challenging application and network scenarios like video conferencing over cellular networks.
%Our experiments also confirm the feasibility of this approach for a wide range of application and network scenarios. %We also evaluate challenging scenarios like the use of video conferencing over cellular networks. 
However, if access capacity is limited, duplication may cause edge congestion, we discuss possible workarounds for reducing sender overhead in ~\S\ref{subsec:deployment}.
}
\end{comment}

%provides high reliability at low cost. It judiciously uses the expensive inter-DC bandwidth to protect against packet losses on the Internet.




%Figure~\ref{fig:solution-space} shows the reliability received by application as a function of its requirement and cost. Ideally, we would like to stay on optimal line, however, both Internet and cloud offer different levels of reliability at different cost.  While the cost of using public Internet paths is less than that of cloud inter-DC paths, there is at least an order of magnitude difference in reliability offered by both~\cite{cloudstudy-www}. On average, loss rate on public Internet paths can go up to 1\%~\cite{fcc_loss,cloudstudy-www}.
%We argue that in current settings, we only need to rely on the cloud whenever the best-effort Internet cannot provide the desired reliability i.e. we can still rely on public Internet to deliver most (\textasciitilde99\%) of the packets on time and use cloud to augment end-to-end availability. 

%We propose \emph{judicious} use of cloud paths: leveraging the availability and performance of cloud only when the best-effort Internet encounters problems. Our proposed packet recovery service provides high reliability at low cost and judiciously uses the expensive inter-DC bandwidth to protect against packet losses on the Internet.

%Figure~\ref{fig:solution-space} shows the reliability received by application as a function of its requirement. Ideally, we would like to be on the optimal line. However, public Internet paths provide average reliability at low cost. Cloud paths, on the other hand, offer high reliability at much higher cost. We believe that with current cloud costs and availability of Internet paths, it is not feasible to send all of the user's traffic through cloud overlay and not use public Internet at all.

%We argue that in current settings, we only need to rely on the cloud whenever the best-effort Internet cannot provide the desired reliability. We propose \emph{judicious} use of cloud paths: leveraging the availability and performance of cloud only when the best-effort Internet encounters problems. Our proposed packet recovery service provides high reliability at low cost. It judiciously uses the expensive inter-DC bandwidth to protect against packet losses on the Internet.

%We now present a potential cloud based packet recovery service %that can be deployed in network in many different ways.
%Our proposed packet recovery service judiciously uses the expensive inter-DC bandwidth to protect against packet losses on the Internet. 

\begin{comment}

\begin{figure}[!t]
 \centering
 \includegraphics[width=1.6in]{figures/solution-space.png}
 \caption{Reliability Solution Space Analysis}
 \label{fig:solution-space}
\end{figure}

\end{comment}
\begin{comment}


We now outline few basic approaches that can use cloud overlay in a cost effective manner. 

\emph{Reactive}. A sender only uses cloud overlay when public Internet path degrades or suffers from an outage (Fig~\ref{fig:reactive}).
There are two main problems this scheme, first, initial lost packets, that trigger path switchover, will not be recovered within acceptable time for the application. Second, deciding when and how long to use cloud overlay is not trivial. 

%If losses are short, switching late provides no benefit.
%switching early when loss period is short will increase overlay cost whereas a late decision will result in poor quality of experience. 

\emph{Corrective}. In this scheme, only coded packets are sent on cloud path and all the data packets go through public Internet path (Fig~\ref{fig:corrective}). While, the chance of losing coded packet is very low on cloud paths, the problem of coping with bursty losses and outages remains.

\emph{Proactive}. A copy of data packet is sent to data center, where it is stored and only sent to receiver when needed (Fig~\ref{fig:proactive}). This scheme takes advantage of current cloud pricing model, where incoming traffic is free and outgoing is charged. However, not only it doubles the sender overhead but also requires a two node overlay for effective performance, hence increasing the cloud bandwidth costs. 

If a single DC overlay is used for packet storage and recovery then overlay will not provide timely packet recovery.
For example, if the DC node near to the sender is used then receiver will have to go all the way back to sender's region for recovery, resulting in higher recovery times. Similarly, if a DC closer to receiver is used then losses on sender-DC path and their subsequent recovery will dominate packet recovery times. If a DC in the middle is used, it will combine worst of both scenarios as both sender-DC and receiver-DC paths will have relatively high RTTs. In a two node overlay, one DC is closer to sender and other is closer to receiver. Sender to cloud losses are recovered in short amount of time (using traditional ARQ based schemes) and receiver can easily recover lost packets by querying its nearest cloud node. However, high cost of using inter-DC bandwidth for \emph{all} data packets will render this scheme unfeasible.


\emph{Hybrid}. \sys{} uses a modified proactive scheme, instead of sending all packets from sender's DC to receiver's DC, we only send two different type of coded packets. Our coding scheme not only keeps inter-DC cost low but also recovers from losses within half RTT. However, \sys{}'s proposed design doubles the sender overhead. We now discuss various deployment scenarios that reduce this overhead and make \sys{} a feasible solution. 


%In our scheme, a two node cloud overlay is used. Senders send copy of their packets to their nearest cloud node. This node combines packets from various senders on the fly and generates coded packets. These coded packets are sent to cloud node near to the receiver and stored for a short time. When a receiver requires packet recovery, its nearest cloud node uses coded packets to generate data packet and sends it to recover. Any losses on sender-cloud and receiver-cloud paths can be recovered using ARQ like scheme. The cost of inter-DC bandwidth is kept low by coded packets. Our coding scheme also copes well with bursty losses and outages.


\paragraph{Deployment Scenarios.} A packet recovery service can be used in variety of ways: it can potentially be deployed by the cloud infrastructure provider, an ISP, or a third-party service provider who pays the cloud operator only for the infrastructure usage. Users can explicitly opt into using it if they require a more reliable packet recovery service -- for example, implemented as a paid service or added value proposition.  
These deployment scenarios determine \emph{who} duplicates the packets (and sends them to the packet recovery service) and \emph{which} packets are duplicated. Three possible scenarios could be:


\begin{enumerate}[leftmargin=*]
    \item \emph{Full Duplication at Source.} This is the primary scenario that we focus on in this paper -- in this case, the source duplicates every packet and sends a copy to the cloud for possible recovery at a later time. 
    Given the relatively low bit rate of many latency sensitive applications, and the increasing capacity of access links, we claim that this strategy is feasible in many common scenarios. 
    Our experiments also confirm the feasibility of this approach for  a wide range of application and network scenarios, including challenging ones like the use of video conferencing over cellular networks. 
    
    
    
    %While it may seem that this overhead of duplication is %excessive, we argue that it is feasible for most of %today's users. There are two main reasons for our claim. %First, many of today's latency sensitive applications have %low bandwidth demands e.g. a Skype HD call only requires %1.5Mbps~\cite{skype_bw}. Second, recent reports have shown %that global average connection speed is increasing and is %at least 7Mbps for both fixed and mobile %users~\cite{akamai_report,speedtest_report}. In fact %Akamai's recent study shows that around 82\% of global %users have at least 4Mbps connection speed with 45\% of %users having greater than 10Mbps~\cite{akamai_report}. 
    
    
    
    \item \emph{Selective Duplication at Source.} When full duplication at source is infeasible -- due to limited access bandwidth or high bitrate of the application -- we can use the packet recovery service 
    only for selected packets, such as an  I-frame for video streaming, important user actions for gaming or AR applications, or the last packet of a window for short TCP transfers~\cite{gentleaggression}. 
    
    %Such selective duplication can provide a lower overhead alternative to the full duplication option described earlier, and can be used in scenarios where sources have limited bandwidth or limited budget for packet recovery. 
    
    \item \emph{Duplication inside the network.} A third strategy, which requires support from the network, involves setting a bit in the packet, which indicates whether packet recovery is required or not. Based on the value of this bit, the ISP could duplicate the packet and send it to the cloud for packet recovery. Similarly, this duplication can also happen at a nearby data center, which can send the original packet through the public Internet and use the cloud path for coded packets only.
\end{enumerate}

Irrespective of which packets are duplicated and who duplicates them, the core of a packet recovery service lies in how the cloud service \emph{encodes} these packets and then subsequently \emph{recovers} them in case of a loss. We now present the design of our proposed packet recovery service, with a focus on these two key design elements. 

\end{comment}
%service,\sys{}, that tries to achieve high reliability while %keeping the cloud bandwidth costs low.

%Once our service receives packets from multiple sources, it %has to decide how to best utilize the inter data center %network to transport these packets to/near their respective %destinations. However, due to cloud bandwidth costs, this %decision is not as simple as forwarding all packets. We now %present design of our proposed packet recovery service,\sys{}, %that tries to achieve high reliability while keeping the cloud %bandwidth costs low.




%\fahad{Perhaps move the discussion around overhead and deployment models (currently in design) to this section}


%
%\john{I don't think we need this.  If we keep it, it has to be its own para:} 
%In the next sections, we describe the design, implementation, and evaluation of \sys{}, a cloud-based wide area packet recovery service for interactive applications.

\begin{comment}


Several factors make it attractive to use cloud as an overlay to support latency sensitive applications. This include: 

\begin{itemize}
    \item \textbf{Lower Latency between end users and DCs.}Using cloud as an overlay provides several benefits that were not possible with traditional overlays ten years ago. One of the major advantages of cloud is their proximity to end users. Cloud providers directly peer with customer ISPs to provider better and faster access to popular web services. Recent studies have also shown that end users are now 1-2 hops away from cloud provider's network~\cite{onehop}~\cite{cloudstudy-www}. Moreover, major cloud providers, Amazon, Microsoft, and Google are currently expanding their global infrastructure at a very fast pace~\cite{aws-locations,azure-locations,google-locations}, essentially reducing cloud latency of millions of end users.

     To get a picture of how fast end users can potentially access cloud infrastructure in the future, we conduct a small study on RIPE Atlas. We randomly select 500 probes (measurement device) around the world and ping websites of three major cloud providers and a CDN provider's network\osama{how long?}. Figure~\ref{fig:cloud-lat} shows that results, we see that \textcolor{blue}{80\%} of users are able to access major services within \textcolor{blue}{50} ms. %We also conduct a small study where we ping these cloud providers using two different US mobile carriers. Figure~\ref{} shows that 50\% of time rtt is less than 70m.  
     These results as well as other studies~\cite{middleboxcloud, rewanhotnets} show that using cloud as an overlay will not add significant latency inflation on end to end path.
    
    \item \textbf{High Reliability of Cloud Paths.}
    Recent measurements show that cloud paths are highly reliable with typical downtime target of few minutes per month~\cite{goog-avail, cloudstudy-www}. In terms of network performance, inter data center paths have an order of magnitude lower loss rates, low jitter and high bandwidth as to compared public Internet paths~\cite{cloudstudy-www}. %\osama{something on cloud connectivity to isp}
   
    %Both Inter-DC, and between ISPs and DCs (mention Azure Direct, etc).
    
    \item \textbf{Ability to support in-network services.} Lastly, cloud infrastructure provides the ability to implement in-network services in software in a scalable and fault tolerant fashion, with the help of network function virtualization)~\cite{combsekar2012,middleboxsherry}. 
    
    %Another advantage of using cloud as a overlay is its performance. A single data center can provide unlimited compute and storage.  (NFV.

\end{itemize}

%\paragraph{Performance of cloud}

\paragraph{Judicious use of the cloud}

While cloud provide significant benefits, one of the major challenges in using cloud overlay is the cost. More specifically, network bandwidth cost of cloud is much higher than compute and storage costs~\cite{amazonprice,azureprice,googleprice}.
Anecdotal evidence, as well as our discussions with operators, suggests that an inter-continental leased line could be an order of magnitude or more expensive compared to a connection to the Internet (which offers no guarantees).
%on the wide area paths). 
This reasoning underlies several recent proposals that try to make efficient use of inter-DC bandwidth in order to reduce their network costs~\cite{rewanhotnets,interdcpricing2016,netstitcher2011}.
Therefore, we characterize the properties of cloud paths in terms of network conditions and cost, and ask the following question: can the cloud be leveraged in a cost-efficient way to make up for the Internet's performance flaws?
%While cloud providers do not charge for incoming traffic, all of the outgoing traffic is charged regardless of its destination.
%In order to reduce bandwidth costs and increase utilization, recent proposals try to make efficient use of inter data center bandwidth~\cite{rewanhotnets,interdcpricing2016,netstitcher2011}.
%\fahad{Needs to be beefed up, citework that is motivated by WAN cost}

%\paragraph{Judicious use of the cloud }


We argue that in current settings, we only need to rely on the cloud whenever best-effort public Internet cannot provide the desired quality of service. We propose judicious use of cloud paths: leveraging the availability and performance of clouds only when the best-effort Internet encounters problems. Our goal is to achieve network performance of cloud paths while keeping the costs low. 


In the next sections, we describe the design, implementation, and evaluation of \sys{}, a cloud-based packet recovery service.
\end{comment}









\begin{comment}
\osama{start of sigcomm writeup}
%\osama{section: how skype performance varies with network conditions, why using cloud is better, advantages/disadvantages %of cloud, judicious use of cloud}

In this section, we show how poor network conditions can affect interactive applications such as Skype (\ref{subsec:skype-motiv}),
and how using the cloud as an overlay can potentially improve QoS of interactive applications over wide area paths, but why such paths need to be used in a judicious manner to maintain cost-effectiveness (\ref{subsec:cloud-motiv}).

\subsection{Limitations of Today's Internet}
\label{subsec:skype-motiv}

%Traditionally, the best-effort service of the Internet has been able to keep pace with the massive growth of applications in scale and %complexity. However, network performance can still be insufficient for certain classes of applications and environments, especially interactive %applications across wide area networks.

\paragraph{Network performance impacts QoE.}
Several recent studies show how poor network conditions impact the user experience for video and interactive applications. For example, a recent study~\cite{via2016} of 430 million Skype calls reveals that network conditions such as round trip time (RTT), loss rate, and jitter are directly correlated with perceived user experience. The study shows that wide area paths are particularly prone to poor network conditions, but that a managed overlay architecture consisting of globally distributed relays can significantly improve network performance and, consequently, user QoE. For example, carefully assigning a subset of calls to use the relay path can improve Skype audio call quality by 45\%. 

\paragraph{QoE can be poor despite aggressive FEC.}
Applications like Skype use aggressive redundancy techniques to cope with packet losses. We conduct an experiment to understand the benefits of Skype's forward error correction (FEC) mechanism under poor network conditions that are typically observed on wide area paths.

We conduct measurements using two nodes with an emulated wide area path between them (similar to the methodology used by Zhang et al.~\cite{zhang2012profiling} and further described in Section~\ref{subsec:skype-perf}). We run Skype video calls  while varying network parameters such as RTT, loss rate, and jitter, and measure the resulting objective quality of video.

Our experiments show that Skype's use of FEC is aggressive, even when packet loss rates are low, yet effective in correcting only 
%\john{uniformly random is the wrong word -- that is what happens in a model, never in real life.}
intermittent packet losses. %even up to packet loss rates around 10\%. For these types of losses, FEC is enough to maintain consistent 
Previous measurement studies as well as our experiments show that wide area paths often experience bursty losses or even outages that can last for seconds~\cite{ron, rewanhotnets}. Our experiment shows that under such worst case scenarios,  Skype's FEC mechanism is insufficient to maintain an acceptable level of QoE based on the peak signal-to-noise ratio (PSNR) as shown in Figure~\ref{fig:skype-outage}. 
% These technicalities are better described in the evalation section.
%\john{opaque text.  I'm guessing structural similarity is a quality metric?}
%(Similar results using structural similarity QoE metrics are omitted.)
In these cases, the number of frames with poor PSNR scores (less than \textasciitilde30) significantly increases, degrading the video quality with pixelation and frozen video. For some applications, such as trying to watch the last few crucial minutes of an important basketball game in New York from India, or trying to conduct a job interview from Boston with an applicant in Australia, these conditions are unworkable. There are many similar scenarios in which this tail performance of the wide area Internet is unacceptable for services like Skype video, and it more broadly presents a barrier to harnessing the full potential from an emerging class of next-generation applications such as networked VR and remote telesurgery.



%\osama{More details about how skype works and figure with results showing skype bad
%performance with varying loss rates and jitter/latency}

\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.16]{graphs/skype_motivation.png}
 \caption{PSNR scores from two minute Skype video conferences as loss rate varies. During a 30 second outage, video quality suffers and the PSNR of affected frames degrades considerably more than even high rates of independent losses.}
 \label{fig:skype-outage}
\end{figure}

\end{comment}

\begin{comment}
\begin{figure}[!t]
 \centering
 \includegraphics[scale=0.18]{graphs/psnr-cdf2.png}
 \caption{PSNR scores from two minute Skype video conferences as loss rate varies. During outages, video quality suffers and the PSNR of affected frames degrades considerably more than even high rates of independent losses.}
 \label{fig:skype-outage2}
\end{figure}
\end{comment}


\begin{comment}
\subsection{A Case for Cloud Paths}
\label{subsec:cloud-motiv}
%\fahad{Text needs to be updated.}\osama{updated now} 
Given the limitations of the best effort Internet paths for the interactive applications of today and tomorrow, we consider the cloud as a potential solution. Some interactive applications, such as Skype and Google Hangout,
% JB:  just Hangout
are already migrating their services to at least partial use of cloud relays~\cite{via2016}, but there has been little work in studying how to best utilize the cloud for these types of interactive communications. Therefore, we characterize the properties of cloud paths in terms of network conditions and cost, and ask the following question: can the cloud be leveraged in a cost-efficient way to make up for the Internet's performance flaws?

\paragraph{Advantages of the Cloud as an Overlay:}

%\paragraph{Wide-area Cloud Paths are Highly Available.}
There are several advantages of using the cloud as an overlay. First, measurements show that cloud paths are highly reliable with typical downtime target of few minutes per month~\cite{goog-avail, interdcpathstech2016}. 
%A recent measurement study shows that wide area cloud paths have availability of three 9's whereas average Internet paths have %availability of only two 9's~\cite{interdcpathstech2016}. 
Second, cloud operators also strive to provide low latency access to various services to end users. They directly peer with customer ISPs to provider better and faster access to popular web services~\cite{goog-onehop}. Hence, using cloud paths does not incur significant latency inflation~\cite{middleboxcloud, rewanhotnets}.
Third, cloud infrastructure provides the ability to implement in-network services in software in a  scalable and fault tolerant fashion, with the help of network function virtualization (NFV)~\cite{combsekar2012,middleboxsherry}.  

%Hence, by using a data center as an overlay node, we can implement .\osama{this needs improvement}

\paragraph{Cost of the Cloud:}
Although the cloud as an overlay provides significant benefits, it can be expensive to use, especially due to the high cost of inter-DC bandwidth.
Anecdotal evidence, as well as our discussions with operators, suggests that an inter-continental leased line could be an order of magnitude or more expensive compared to a connection to the Internet (which offers no guarantees on the wide area paths). 
This reasoning underlies several recent proposals that try to make efficient use of inter-DC bandwidth in order to reduce their network costs~\cite{rewanhotnets,interdcpricing2016,netstitcher2011}. 
%Similarly, making efficient use of the wide aSeveral WAN optimization techniques like compression, de-duplication, and FEC are used to reduce %cost and increase utilization. Hence, a cloud based overlay service will incur significant bandwidth costs.

\paragraph{Judicious use of the cloud.}
We argue that in current settings, we only need to rely on the cloud whenever best-effort public Internet cannot provide the desired quality of service. We propose judicious use of cloud paths: leveraging the availability and performance of clouds only when the best-effort Internet encounters problems. In the next sections, we describe the design, implementation, and evaluation of \sys{}, a cloud-based wide area packet recovery service for interactive applications.

\osama{end of sigcomm writeup}
\end{comment}










==> ReWAN-arxiv(1)/related-work.tex <==
\section{Related Work}
\label{sec:related-work}
\begin{comment}
Divide into following categories

\begin{itemize}
    \item General overlays (RON, One hop source routing, MONET, Brocade, OverQoS)
    \item Using cloud as overlay (CRONets, VIA)
    \item Recent similar works in improving QoS (ARROW, RPT, BW guarantees)
    \item Coding techniques (Maelstrom, RPT)                        
\end{itemize}
\end{comment}

\sys{} connects to and benefits from a large body of prior work. We comment on key pieces from the literature that our most relevant to our study.

\textbf{Overlay Networks.} Our work is inspired by \emph{overlay} networks that improve availability by using detour points, e.g., RON~\cite{ron}, one-hop source routing~\cite{detour}, Spines~\cite{spines}, etc. Our use of the cloud as an overlay creates unique opportunities and challenges. For example, we can do sub-RTT recovery, but to minimize cost, we have to send an additional small number of recovery packets. 
Individual aspects of \sys{}'s design also resonate with other overlay based solutions. 
For example, applying coding across users is similar to applying QoS across streams~\cite{overqos}.
Recently, there have been proposals that make the case for using cloud as an overlay to support interactive applications (VIA~\cite{via2016})%, ReWAN~\cite{rewanhotnets}) 
, TCP-based applications (CRONets~\cite{cronets2016}), as well as delay tolerant applications~\cite{ccr-slack}. 
Schemes like VIA improve performance by routing \emph{all} of a certain user's traffic through the overlay path. Our evaluation shows that \sys{} can achieve similar benefits while only sending a fraction of traffic over the expensive inter-DC paths. Finally ReWAN~\cite{rewanhotnets} provides a high level idea of using coded packets across the cloud paths for packet recovery. In this paper, we provide a complete design, including a tunable coding algorithm and recovery protocol, as well as deployment and evaluation under realistic network conditions as well as under controlled environments. 
%ReWAN\cite{rewanhotnets} provides a high level idea of using coded packets across the cloud paths for packet recovery. We provide a complete design, including a tunable coding algorithm and recovery protocol, as well as deployment and evaluation of \sys{} under realistic network conditions. 

%\sys{} is primarily inspired by overlay networks that were popular more than a decade ago
%(e.g., RON~\cite{ron}, MONET~\cite{monet}, one-hop source routing~\cite{detour}, Spines~\cite{spines}, etc). These networks use detour points to %improve network reliability, whereas \sys{} uses cloud infrastructure, which presents unique opportunities and challenges. For example, \sys{} cannot %fully utilize cloud paths due to high cost and sends only small number of packets. While traditional overlay nodes are constrained by limited %processing power and storage, \sys{}'s overlay node is essentially the whole data center with \emph{infinite} resources. Using data center node as %overlay is also similar to super peers in overlay networks~\cite{landmarkoverlay} except \sys{}'s cloud nodes are connected through dedicated paths. In %terms of QoS, \sys{}'s use oof coding across users is similar to applying QoS across streams~\cite{overqos}.





\begin{comment}

\fahad{reusing text from hotnets} \\

\textbf{Overlay Networks.} Our work is inspired by \emph{overlay} networks that improve availability by using detour points (e.g., RON~\cite{ron}, MONET~\cite{monet}, one-hop source routing~\cite{detour}, Spines~\cite{spines}, etc). Our use of cloud as an overlay creates unique opportunities and challenges. For example, we can do sub-RTT recovery, but to minimize cost, we have to send a small number of recovery packets. Individual aspects of \sys{}'s design also resonate with other overlay based solutions. 
For example, our use of DCs as overlay nodes has similarities with super peers in overlay networks~\cite{landmarkoverlay}:  DCs can be viewed as super peers with dedicated links between them, with cost associated with the use of these links  (and other resources). Similarly, applying coding across users is similar to applying QoS across streams~\cite{overqos}. 

\textbf{Cloud Overlays.}(CRONets, VIA, ReWAN-HotNets)
\end{comment}

%\textbf{Cloud-based Services.} To leverage the advantages of the cloud, various proposals have argued for moving a wide range services to the cloud. 
%This include proposals for moving middlebox functionality~\cite{middleboxcloud} or disaster recovery to the cloud~\cite{disastercloud}. 
%We argue for using cloud in a judicious manner to provide richer network services that complement the best effort service of IP. 

%\osama{this category copied from hotnets} \\


%\begin{comment}


\textbf{Inter-Data Center Networking.} Our work complements the large body of work on \emph{inter-data center} networking. This includes application of software defined networking (SDN) to such environments (e.g., SWAN~\cite{swan}, B4~\cite{swan}), as well as techniques that meet specific workload needs (e.g., application deadlines~\cite{eurosys15, tempus}). Similarly,  studies on inter-DC measurements~\cite{cloudcmp, eurosys15} have mainly focused on inter-DC \emph{bandwidth}. \sys{}'s use of inter-DC paths to send coded packets for recovery is complementary to these prior efforts. 

%\end{comment}
\textbf{Coding and Cooperative Recovery.}
Traditionally, network coding techniques have seen widest use in  the context of wireless networks~\cite{Katti06,networkcoding2006}. 
%describe methods for reducing retransmissions, recovering from packet loss, and  improving throughput.  
\sys{} applies cross-stream coding on wide area Internet paths and uses it to recover lost packets.
FEC based coding schemes have also been used in different contexts over the last several decades. The most relevant work to our scheme is Maelstrom~\cite{maelstrom}, which uses an FEC-based technique to reduce packet loss on lambda networks. Maelstrom's layered interleaving provides additional protection against bursty losses, but at the expense of higher decoding delay, which limits its use for highly interactive applications. Also, unlike Maelstrom,  the coded and data packets are sent on \emph{different} paths, with very different properties. 


%While we send FEC packets across the data center paths -- these packets provide protection against losses on the public Internet path instead of losses on the inter-DC path. In terms of packet recovery, Maelstrom's recovery latency depend on the size of the burst. Hence, it is not useful in large bursty and outage scenarios.

%Network coding has also been proposed for distributing content ~\cite{gkantsidis2005network}. \sys{} provide packet recovery for interactive applications and does not use cloud overlay for content distribution.

%Networking Coding. Typical use - wireless, content distribution. 


%We do not recover packets on inter data center paths and our use of 
%network coding along with FEC to recovery Public Internet path losses on wide area is different and unique.

%\osama{this category copied from hotnets} \\
\textbf{Reliable and Low Latency Wide Area Communication.} Finally, we share the goals of proposals that call for \emph{low latency and high reliability} for wide area communication~\cite{speedoflight, arrow, caip, npp}. For example, Arrow~\cite{arrow} is proposed as a reliable, wide area service;  it uses reliable paths as tunnels to improve end-to-end reliability. While inter-DC paths are likely to have similar properties as Arrow's reliable paths, our approach of only using these paths for recovery is different and complementary to Arrow's goals. 
%Multipath TCP~\cite{mptcp-acm} uses WiFi and 3G paths to split traffic and provide high throughput whereas \sys{} duplicates packets on cloud path to provide high reliability. Recently, there also have been some proposals that exclusively improve performance of TCP short %flows~\cite{ietf-tcpm-rack, tcpm-tcp-loss-probe} using different techniques (e.g. per packet timestamps, early retranmsissions etc).We, however, use nearest DC to recover lost packets. 



%Multipath TCP~\cite{mptcp-acm} offers a redundant scheduler that sends copy of packet through an alternate path. It can replace \sys{}'s sender module but would require major changes to support UDP traffic, coding, and recovery. Recently, there also have been some proposals that exclusively improve performance of TCP short flows~\cite{ietf-tcpm-rack, tcpm-tcp-loss-probe} using different techniques (e.g. per packet timestamps, early retranmsissions etc). We, however, only view \sys{}'s tcp performance as an additional benefit. 



%Compare with Via -- Does Via have a more narrow scope (just Skype audio)? Via requires application to contact management controller before starting service. In Via, flow is completely on a single, chosen path, unlike in ReWAN.


